Towards a theory of out-of-distribution learning

Learning is a process wherein a learning agent enhances its performance through exposure of experience or data. Throughout this journey, the agent may encounter diverse learning environments. For example, data may be presented to the leaner all at once, in multiple batches, or sequentially. Furthermore, the distribution of each data sample could be either identical and independent (iid) or non-iid. Additionally, there may exist computational and space constraints for the deployment of the learning algorithms. The complexity of a learning task can vary significantly, depending on the learning setup and the constraints imposed upon it. However, it is worth noting that the current literature lacks formal definitions for many of the in-distribution and out-of-distribution learning paradigms. Establishing proper and universally agreed-upon definitions for these learning setups is essential for thoroughly exploring the evolution of ideas across different learning scenarios and deriving generalized mathematical bounds for these learners. In this paper, we aim to address this issue by proposing a chronological approach to defining different learning tasks using the provably approximately correct (PAC) learning framework. We will start with in-distribution learning and progress to recently proposed lifelong or continual learning. We employ consistent terminology and notation to demonstrate how each of these learning frameworks represents a specific instance of a broader, more generalized concept of learnability. Our hope is that this work will inspire a universally agreed-upon approach to quantifying different types of learning, fostering greater understanding and progress in the field.

==> content_jmlr.tex <==
\input{text/0_abstract}

\input{text/1_introduction} %\clearpage
% \input{text/2_prelims} %\clearpage
\input{text/2_framework} %\clearpage
\input{text/3_learnability}
% \input{text/5_super} %\clearpage
\input{text/4_theoretical_results} %\clearpage
\input{text/5_supertasks} %\clearpage
\input{text/6_discussion} %\clearpage

% \clearpage
\bibliography{biblifelonglearning.bib}




% \appendix
% %  
% \clearpage
% % \input{text/algorithms}
% \input{text/machine_learning}
% \input{text/learning_tasks}
% \input{text/framework} %\clearpage
% \input{text/bio_learning}
% % \input{text/learning_def}

==> extra/algorithms.tex <==



\section{Learner Evaluation}
\label{app:algorithms}


Thus far we have an introduced a task framework that elucidates precisely what is a task. We then extended this framework to describe various settings such as transfer learning, multitask learning, etc. The next logical step now is establishing evaluation criteria for learners in these various contexts.    
\subsection{Learner Efficiency}
    The next logical question is: which learner is better? Learning efficiency dealt with the question of whether we learn better with $\D_A$ or $\D_B$ given a learner $f$. Now we flip the question, do we learn better with learner $f$ or learner $f'$ given the data $\D$?
    \begin{definition}[Learner Efficiency]
        Given a task $t$ and two learners $f, f' \in \mc{F}$, along with a data $\D$, the learner efficiency is defined as
        \begin{align*}
            AE_{\D}(f, f') = \frac{\mc{E}_{f}(\D)}{\mc{E}_{f'}(\D)} 
        \end{align*}
    \end{definition}
    If $AE > 1$, then learner $f'$ is a "better" learner and vice versa. The learner efficiency is indeed very \comE{related?  (missing word)} to the learning efficiency. They are both ratios of (centered) generalization errors.
\subsection{Other Metrics}
The goal of this section is to demonstrate the wide applicability of the concept of learning efficiency.

\subsubsection*{Few-Shot Learning}
\citet{Wang2020} define few-shot learning as a "type of machine learning problem" which "contains only a limited number of examples". In our framework, this corresponds to a task $t$ with data $\D_n$ where $n$ is small. Due to the limited availability of data, we use data from other tasks and hope that this data helps us learn a better hypothesis. This is exactly a meta-learning \comE{transfer learning?} problem then, and so we can use the meta-learning framework. Assume all the definitions and quantities from section \ref{sec:meta_learning}. Recall the meta-learning metric,
\begin{align*}
    \sum_{j = k + 1}^{n}\LE_f^j(\D^j, \D \cup \D^j )\cdot p(j).
\end{align*}
In few-shot learning, $k + 1 = n$ (i.e. we only have one unseen task we care about) and so the metric becomes
\begin{align*}
    \LE_f^n(\D^{n}, \D \cup \D^n).
\end{align*}
The only other component to few-shot learning is that $\abs{\D^{n}}$ is small. If $\LE_f^n(\D^{n}, \D \cup \D^n) > 1$, then we have successfully utilized the out-of-task data to learn a better hypothesis in a low data context.
\subsubsection*{Continual Learning Metrics}
Assume we have a lifelong learning environment $\mc{T}$ with $n$ tasks, and a data sequence $\D_n$. Assume also that the Bayes risk $R^* = 0$ for all tasks in $\mc{T}$. \citet{Rodríguez2018} introduces the following three metrics for a lifelong learner $f$,
    \begin{enumerate}
        \item Accuracy:
        \begin{align*}
            \frac{1}{\frac{n(n + 1)}{2}}\sum_{i \geq j}^{n}\mathcal{E}^{j}_f(\D^{< i})
        \end{align*}
        \item Backward Transfer:
        \begin{align*}
            \frac{1}{\frac{n(n - 1)}{2}}\sum_{i = 2}^{n}\sum_{j = 1}^{i - 1}\mathcal{E}^{j}_f(\D^{< i}) - \mathcal{E}^{j}_f(\D^{< j})
        \end{align*}
        \item Forward Transfer:
        \begin{align*}
            \frac{1}{\frac{n(n - 1)}{2}}\sum_{i < j}^{n}\mathcal{E}^{j}_f(\D^{< i})
        \end{align*}
    \end{enumerate}
    These measures can recast in terms of learning efficiency by multiplying and dividing each quantity by $\mc{E}_f^j(\D)$,
    \begin{enumerate}
        \item Accuracy:
        \begin{align*}
            \frac{\mathcal{E}_f^j(\D)}{\frac{n(n + 1)}{2}}\sum_{i \geq j}^{n}\LE_f^j(\D^{< i}, \D)
        \end{align*}
        \item Backward Transfer:
        \begin{align*}
            \frac{\mathcal{E}_f^j(\D)}{\frac{n(n - 1)}{2}}\sum_{i = 2}^{n}\sum_{j = 1}^{i - 1}\LE_f^j(\D^{< i}, \D) - \LE^{j}_f(\D^{< j}, \D)
        \end{align*}
        Notice that $LE^{j}_f(\D^{< j}, \D)$ is the backward efficiency of $f$ for task $t_j$.
        \item Forward Transfer:
        \begin{align*}
            \frac{\mathcal{E}_f^j(\D)}{\frac{n(n - 1)}{2}}\sum_{i < j}^{n}\LE^{j}_f(\D^{< i}, \D)
        \end{align*}
    \end{enumerate}
    
\comE{This section is a bit disconnected.}

\comE{It seems odd to separate the continual learning metrics from the lifelong learning metrics, when earlier the paper said they were two names for the same thing. I personally consider them a bit differently, in that continual learning (focusing on continually updating a model to learn multiple consecutive tasks) is a key component of lifelong, but that lifelong involves much broader reasoning about what tasks are still current, goal-direction, learning from interaction, etc.}

\subsubsection*{Lifelong Learning Metrics}
We presented forward and backward efficiencies as the relevant metrics for lifelong learning in section \ref{sec:lifelong}. There are also other metrics, in addition to the continual learning ones above, that merit mention. Let $\D_{< i}$ be the sequence of data points up to and including the $i$th data point. Also let $\D_{< i}^j = \{(D_k, J_k): (D_k, J_k) \in \D_{< i}, J_k = j\}$ be the set of data points up to and including the $i$th data point which are from task $t_j$. 
\begin{enumerate}
    \item \textbf{Performance recovery},
    Recall that $\D_n$ is the concatenation of data batches $\D_{A_1}, \D_{A_2}, $etc. For each data point $(D_i, J_i)$ in $\D_{A_k}$, notice that it has an absolute position/index $i_{abs}$ in $\D_n$ and a relative position/index $i_{rel}$ in $\D_{A_k}$. 
    Consider the last data point in $\D_{A_1}$, and assume it has index $i_{min}$. Now, for each subsequent data batch, calculate
    \begin{align*}
        \mathbf{I}_{\D_{A_k}} = \{i_{rel}: (D_{i_{abs}}, J_{i_{abs}}) \in D_{A_k}, \LE_f^j(\D_{< i_{abs}}, \D_0) \geq \LE_f^j(\D_{< i_{min}}, \D_0)\}.
    \end{align*}
    This set, for a data batch $\D_{A_k}$ is the set of indices for which the learning efficiency is greater than the terminal first batch learning efficiency $LE_f^j(\D_{<i_{min}}, \D_0)$. Now construct the set 
    \begin{align*}
        \{\big(k, \min\mathbf{I}_{\D_{A_k}}): k \in \mathbb{N}, \D_{A_k}\text{ is a data batch}\big)\} \enspace. \mbox{\comE{Whenever you have a non-inline equation followed by a period, it's good form to use enspace before the period to ensure proper spacing.  Applies to the whole document.}}
    \end{align*}
    Intuitively, the above set represents how fast the lifelong learner $f$ recovers performance whenever the task is changed. The slope of the least squares line fit to the points in the above set represents the performance recovery metric.
    \item \textbf{Performance maintenance},
    Consider a task $t_j$. Let $\mathbf{I}_j = \{i: J_i = j, J_{i + 1} \neq j\}$ be the set of indices of data points where the current data point is from task $t_j$ but the next one is not. Then performance maintenance is defined as
    \begin{align*}
        \text{median}\{\LE_f^j(\D_{< i}, \D_0): i \in \mathbf{I}_j\} - \LE_f^j(\D_{< \min\mathbf{I}_j}, \D_0).
    \end{align*}
    Intuitively this quantity measures how much performance $f$ retains on $t_j$ as it encounters new tasks.
    \item \textbf{Performance relative to a single task expert}.
    Consider a task $t_j$. A single task expert is a learner trained on only target task data. For example, the learner can be trained on only task $t_j$ data.  Let $\mathbf{C}_j = \{i: (D_i, J_i) \in \D_n, J_i = j\}$ be the set of indices of data points which correspond to task $t_j$. Then, performance relative to a single task expert is defined as
    \begin{align*}
        \frac{\sum_{i \in \mathbf{C}_j}\LE_f^j(\D_{< i}, \D_0)}{\sum_{i \in \mathbf{C}_j}\LE_f^j(\D_{< i}^j, \D_0)}.
    \end{align*}
    Intuitively this represents how much better a lifelong learner is better than a single task learner.
    \item \textbf{Sample efficiency}.
    Let $LL$ be short for lifelong and $STE$ be short for single task expert. Consider the functions $g^j_{LL}$ and $g^j_{STE}$ which given an index $k$ return the rolling average of the learning efficiencies up to that data point respectively for the lifelong learner (trained on all data) and the single task expert for task $t_j$ (learner trained on only $t_j$ data),
    \begin{align*}
        g^j_{LL}(k) & = \frac{1}{k}\sum_{i = 1}^{k}\LE^j_f(\D_{< i}, \D_0), \\
        g^j_{STE}(k) & = \frac{1}{k}\sum_{i = 1}^{k}\LE^j_f(\D_{< i}^{j}, \D_0).
    \end{align*}
    Let $\hat{k}_{LL} = \argmax_{k} g^j_{LL}(k)$ and $\hat{k}_{STE} = \argmax_{k} g^j_{STE}$. Then, the sample efficiency of $f$ is defined as
    \begin{align*}
        \frac{\hat{k}_{STE}}{\hat{k}_{LL}}\cdot\frac{\max_{k}g^j_{LL}(k)}{\max_{k}g^j_{STE}(k)}.
    \end{align*}
    Intuitively this measures how much the lifelong learner is more efficient than the single task learner.
\end{enumerate}
Note that if we assume $R^* = 0$ and scale any learning efficiency by $\mathcal{E}_f^j(D_0)$, we recover metrics in terms of only the generlization error.
\subsubsection{Transfer Benefit Ratio}
\citet{Pearl2012} begins from a principled, statistical basis to explore the question of transfer learning. In an extremely simple setting, a metric that measures the benefit of transferring from out-of-task data is introduced. Specifically, there is a simple, one-dimensional, linear model with parameter $\tau$ of interest, and two other parameters $a, b$ such that $\tau = ab$. The work then explores estimating $\tau$ with just task data, and estimating $ab$ with both task and out-of-task data. The reasoning for this is that the parameter $a$ a priori is known to be the same for the distributions of the task data and the out-of-task data, whereas the parameter $b$ is not. Hence $a$ is estimated with both task and out-of-task data, while $b$ and $\tau$ are not. The estimation technique is ordinary least squares (OLS) for each parameter, but the data used is different.

The work then goes on to compare the variance of the estimators and defines their ratio as the \textbf{transfer benefit ratio}
\begin{align*}
    \frac{var(\hat{\tau}; \D_n^1)}{var(\hat{a}\hat{b}; \D_n, \D_n^1)},
\end{align*}
where $\D_n^1$ is only task data and $\D_n$ is all of the data. Implicitly then, the author has assumed mean squared error as the risk function. Since both estimators are unbiased, the ratio of variances turns out to be a ratio of risks. Furthermore, assuming the data is random (and not fixed as in \cite{Pearl2012}), we rewrite the transfer benefit ratio in the notation of this work as
\begin{align*}
    \frac{\mc{E}_{f_1}(\D_n^1)}{\mc{E}_{f_2}(\D_n)},
\end{align*}
where $f_1$ is OLS estimation of $\tau$ using $\hat{\tau}$ and $f_2$ is OLS estimation of $\tau$ using $\hat{a}\hat{b}$. While not exactly a learning efficiency, it is very close in that it is a ratio of generalization errors.


==> extra/bio_learning.tex <==

\section{Intuitive Explanations of Various Learning Paradigms}
\label{app:bio_learning}

\subsubsection*{Point Estimation}
% \begin{example}[Point Estimation]
    Given a dataset, and we desire to summarize it in a particular way.  Specifically, in point estimation, the goal is to find a generative distribution that characterizes the observed data.  For example, if the data we obtain are heights of individuals that live in the United States, we may desire to know what is the average height. Estimating the average height is an instance of point estimation.  To proceed, we assume each data point is sampled identically and independently (iid) from some true but unknown distribution, and we further assume that the distribution can be parameterized to include the  parameter of interest. Then, we leverage the data to obtain   a ``good'' estimate for the parameter. If the other parameters of the distribution are also provided or estimated, then we could sample from this distribution and generate a new dataset that looks `similar' to the original dataset.  
    % 
    A simple example is estimating the average height of individuals in a particular population. Note that estimating this parameter does not require making a Gaussian, or any other strong modeling assumptions.  Moreover, in general, the data need not be scalars or even multivariate Euclidean data; rather, one can estimate parameters of distributions for arbitrary data spaces, including images and networks. 
    % 
% \end{example}


\subsubsection*{Hypothesis Testing}
% \begin{example}[Hypothesis Testing]
    As with point estimation, we are given a dataset, and we typically assume each datum is sampled iid from some true but unknown distribution. In hypothesis testing, the goal is to decide whether or not the evidence suggests that the data are sampled from some distribution in the ``null hypothesis''.  In general, the null hypothesis can be a set of distributions, for example, all univariate Gaussian distributions. 
    % 
    In the Neyman-Pearson framework of hypothesis testing, one also postulates an ``alternative hypothesis'', which is another set of distributions that is non-overlapping with the null hypothesis. A  valid guess is one which bounds the probability of guessing alternative hypothesis when, under the model assumptions,  the correct answer is null hypothesis (this bound is called the significance level). We desire a procedure that maximizes the probability of guessing alternative hypothesis if the correct answer is in fact alternative hypothesis, that is, has maximum \textit{power} under the model. 
    % 
Crucially, in hypothesis testing, the agent can only take one of two potential actions: reject the null hypothesis, or fail to reject the null hypothesis, but never accept the alternative.  The reason for this is related to the no free lunch theorem~\cite{Wolpert1996-oo} and the arbitrary slow convergence theorem~\cite{Devroye1983-tk}, as will be explained below. 
    % 
            A typical example is testing whether a given treatment in a randomized control trial is more effective than placebo. Another example is determining whether two features, for example height and weight, are correlated or not. 
% 
Biological learning agents can be said to perform hypothesis testing whenever the agent learns to make categorical decisions to no longer accept their previous operating assumptions.  
% \end{example}

\subsubsection*{Supervised Learning}
    % 
    In supervised learning, as before, we have a dataset which is a set of pairs, where each pair is a pattern and the corresponding  label for that pattern.
    The patterns are often represented by feature vectors. When the labels are categorical, we have a classification problem; when the labels are continuous, we have a regression problem.  The labels can be more complicated, including multivariate, images, networks, etc., in which case, the problem is a ``structure learning problem''.  
    Regardless of the feature and label spaces,  we typically assume each pair is sampled iid from some true but unknown distribution. In supervised learning this distribution is a joint distribution over patterns and labels. 
    % 
    The objective with supervised learning is to leverage this data to produce a function that, which when given a pattern, outputs an estimated  label.
    % 
    The art in supervised learning is choosing a procedure to produce a function for the task at hand. 
    % 
    Examples of supervised learning include learning functions such as labeling images to their corresponding animals, or using biomedical images to identify troubling anomalies. Such learning naturally arises in both machine and biological learning contexts. 
% 
% \end{example}

\subsubsection*{Unsupervised Learning}
% \begin{example}[Unsupervised Learning]
    Unsupervised learning is very similar to supervised learning. In both, we learn to summarize patterns with labels, but in unsupervised learning, the labels are not provided.  There are two common types of unsupervised learning. If we desire to summarize patterns with categorical labels, we have a clustering problem; if we desire to summarize patterns with   continuous labels, we have a dimensionality reduction problem. As above, patterns can be arbitrarily complex.  We again typically assume each data point is sampled iid from some true but unknown distribution. The objective is essentially identical to the objective in supervise learning: produce a function that for each data point, it outputs an estimated label. One important distinction from supervised learning is that in unsupervised learning, there is not necessarily a function learned for new points, rather, sometimes we simply learn the values of the labels for the observed points, and not a function mapping new points to their corresponding labels. 



\subsubsection*{Streaming Learning}
% 
Streaming scenarios can be any of the above learning scenarios with one modifications: the learner sequentially updates the hypothesis, rather than learning the hypothesis on one batch of data.  There are two possible reasons to use streaming algorithms.  First, the data itself may be streaming, meaning they arrive sequentially, and we may want to make decisions in real time, rather than waiting for all the data to arrive. 
Second, the learner may have computational bounds, and/or there may be real costs associated with computational overhead. In such scenarios, we may require that that the learner can store and operate on a bounded amount of data, using a bounded amount of time. Such constraints are common when the data themselves are streaming.  However, sometimes they are used primarily for computational efficiency reasons.


% \end{example}
\subsubsection*{Online Learning}
% 
% TODO@JV review to refelct updated defo of streaming
% 
Online learning is similar to streaming learning in that decisions are made sequentially, potentially after each data point arrives, rather than leveraging all the data at once.  Online learning differs from the above ``batch'' learning scenarios in that the restriction that each sample $X_t$ is sampled iid is relaxed; rather, the distribution governing the samples can be time-varying, and even adversarial.  This change makes online learning significantly more difficult than ``iid learning'', and therefore has a complementary set of theoretical and methodological results~\cite{Cesa-Bianchi2006-tv}. Online learning does not necessarily have computation complexity constraints.
% \end{example}



\subsubsection*{Transfer Learning}
Transfer learning was first introduced in the early nineties with an approach using neural networks~\cite{Pratt1993-yn}. Given some task and associated data, called the target task and target data, the goal is to  leverage some additional source dataset as to improve upon performance achievable by only using target data. 
Transfer learning is fundamental to biological learning, and has been observed even in insects~\cite{Giurfa2001-nr}. Since its introduction, a large number of papers have investigated learners that implement various versions of transfer learning~\cite{Pan2010-bv}. Fewer papers have investigated the theory underlying transfer learning, although there are some notable exceptions~\cite{Baxter2000-wv,Ben-David2003-fr,Mahmud2008-lp,Hassan_Mahmud2009-bd, kpotufe, Finn2017-fi, jordan2020}. Some key themes of these contributions involve (1) a formal treatment of the task and data generating process, in which some component (either a notion of representation, a prior over parameters, data, or a hypothesis class) is shared across many tasks, and (2) theoretical measures of relatedness between tasks~\cite{Ben-David2008-tv, Dwivedi2019-hw, Shui2019-tb, Helm2020-iv}. In these works, transfer learning is usually analyzed in the context of supervised learning, or further specialization thereof. Some of the extensions we wish to explore in this work are a criterion for transfer learning that applies to a general class of statistical tasks, as well as a performance measure that, rather than measuring similarity between tasks, measures the degree to which a particular learner leveraged source information to improve target performance.


\subsubsection*{Multitask Learning}

Multitask learning can be seen as an extension or generalization of transfer learning. In multitask learning, there are multiple tasks of interest, and no one task is assigned a ``target'' label.  Rather, the goal is to jointly learn from all data to improve on all tasks. 
In a sense, all the datasets act as source datasets to transfer to all the other datasets/tasks.  Perhaps for this reason, many papers discuss both transfer learning and multitask learning together, for example~\citet{Caruana1997-mm,Baxter2000-wv}. Recent theory on multitask learning has largely focused on learning shared representations~\cite{Maurer2016-qv, Jebara2011-rm}.

\subsubsection*{Lifelong (or Continual) Learning}

Lifelong (or continual) learning~\cite{Chen2018Lifelong} generalizes these ideas of transfer and multitask learning to settings in which the agent learns multiple tasks consecutively, building upon its knowledge over time. Lifelong and continual learning are often used interchangeably, though below we will distinguish between the two in operationally meaningful ways below.
As in sequential (online) learning, data arrives incrementally in a lifelong learning setting. More generally than online learning though, it is not just the distribution of data that might change over time, but the task itself will change. The lifelong learner, therefore, might receive new data with updated task information, or without updated task information even though the task has changed. 
% Tasks may be extrinsic and presented sequentially for training, or implicit as the agent interacts with the environment.  


A number of authors have studied this lifelong learning setting, including those who studied transfer and multitask learning~\cite{Chen2018Lifelong,Thrun1995-qy,Thrun1996-kk,Thrun1998-ze}.  The book entitled ``Learning to Learn''~\cite{Thrun2012-sj} seemed to catalyze a renewed interest in the topic, with many articles dedicated to it since. This includes both algorithmic developments dedicated to improving empirical performance on lifelong learning tasks~\cite{ruvolo2013ella,Ruvolo2013-nu,Balcan2015-ao}, as well as many theoretical investigations~\cite{Pentina2014-hl,Pentina2015-xx}.  The recent theoretical investigations mostly focus on sequentially learning shared representations. In other works these problems are referred to as continual learning~\cite{Ring1997-ar}, or online meta-learning~\cite{Finn2019-yv}.  More recent works on continual learning~\cite{Parisi2018Continual,DeLange2019Continual} have focused on updating models to learn new tasks while still retaining performance on all previously learned tasks, thereby avoiding catastrophic forgetting.  Note this may be an inappropriate expectation in some applications, depending on how tasks are defined, since environmental changes over time may render particular tasks obsolete, necessitating forgetting.







==> extra/extra.tex <==
%%% MULTITASK ASYMPTOTICS

% Similar to Section \ref{sec:formal_transfer}, we have basic asymptotic criteria as well.
% \begin{definition}[Multitask Consistency]
%     Learning rule $ (f) $ is weakly multitask consistent (for $P$) if
%     \begin{align*}
%         \liminf_{n \rightarrow \infty}         \E{T}{\TE^T(f)} \geq 1.
%     \end{align*}
%     $ (f) $ is strongly multitask consistent (for $P$) if for all $t \in \mc{T}$,
%     \begin{align*}
%         \liminf_{n \rightarrow \infty} \TE^t(f) \geq 1.
%     \end{align*}
%     Learning rule $ (f) $ is universally weakly (strongly) multitask consistent if it is weakly (strongly) multitask consistent for all $P$.
% \end{definition}

%%% ONLINE LEARNING AND REINFORCEMENT LEARNING

% \subsubsection{Online Learning}

% Online learning refers to a setup in which prediction and learning are intertwined among multiple ``rounds". In each round, the agent is expected to both submit a prediction and update its hypothesis, thereby learning while  deployed. We desire agents that learn efficiently, in the sense that they quickly approach hypotheses with few errors. Formally, in the online supervised learning setting, let $\mc{X}$ be an input space, and $\mc{Y}$ be a label space. Let $\mc{H} \subseteq \{h: \mc{X} \rightarrow \mc{Y}\}$ be some class of hypotheses. Let $\ell: \mc{Y} \times \mc{Y} \rightarrow \mbb{R}_{\geq 0}$ be a loss function. A learning algorithm, also referred to as an agent, 
% % TODO i'm not sure we want 'agent' here'.  agent sometimes also includes, eg, the robot.  and then we have computational issues.  i'd stick with algorithm or learner.
% $f: \mc{H} \times \mc{X} \times \mc{Y} \rightarrow \mc{H}$ consumes a ``current" hypothesis and data point and produces the hypothesis for the next round. $f$ is subjected to $T$ rounds. In round $t$, the following occur.
% \begin{enumerate}
%     \item A data point $(x_t, y_t) \in \mc{X} \times \mc{Y}$ is generated.
%     \item $x_t$ is given to the agent $f$, and it submits the prediction of its current hypothesis $h_t: \mc{X} \rightarrow \mc{Y}$, with the intention that $h_t(x_t)$ is close to the unseen $y_t$.
%     \item $y_t$ is revealed to the agent, and it incurs loss $\ell(h_t(x_t), y_t)$.
%     % TODO i'm not sure y_t is revealed, rather, just the loss is revealed, right?
%     \item The agent updates the hypothesis $(h_t, x_t, y_t) \mapsto h_{t+1}$.
% \end{enumerate}
% % TODO i don't think i'd use t and T here, since we use them later for tasks.  maybe n and N?
% After $T$ rounds, the agent has encountered the sequence $\mc{D}_T = (x_1, y_1), ..., (x_T, y_T)$. At this point, no assumptions have been made on $\mc{D}_T$, nor has the objective of the agent been specified. This is where online learning diverges into a statistical and non-statistical view.

% In the statistical view, the sequence $\mc{D}_T$ is a stream of i.i.d. realization from a fixed, unknown distribution $(X, Y) \iid P_{X, Y}$. The agent considers a specific class of hypotheses $\mc{H} \subseteq \{h: \mc{X} \rightarrow \mc{Y}\}$. Its goal is to find $h \in \mc{H}$ that makes $R(h) = \mbb{E}[\ell(h(X), Y)]$ small, without incurring too much cumulative expected  loss as the rounds progress. That is, the learning algorithm $f$ wishes to minimize regret $\mc{R}^{\text{S}}_T$.
% \begin{align*}
%     \mc{R}^{\text{S}}_T(f) &= \E{}{ \sum_{t=1}^T l(h_{t}(X_t), Y_t)}
% \end{align*}

% % TODO let's introduce the infemum when we need it, which is here, not above.
% In the non-statistical view, the sequence $\mc{D}_T$ is not necessarily assumed to be realized from some distribution, but can be any, even adversarially chosen, sequence. The only way for the agent to ``learn" is by the advice of $N$ experts $h_{i, t}: \mc{X} \rightarrow \mc{Y}$ for $i \in [N]$. Experts output a prediction, but have access to some additional side information at each round $t$ that is unobserved by the agent. The non-statistical view further diverges into the deterministic and randomized scenarios. 

% % TODO i try to avoid "usually" unless it can be qunatified and cited.
% In the deterministic scenario, the agent outputs a single prediction. In classification, this is usually the class outputted by majority of the experts, whereas in regression, it is usually a a weighted average of the expert predictions. Letting $\hat{y}_t$ be the round $t$ prediction, the agent incurs loss $\ell(\hat{y}_t, y_t) = \ell(h_t(x_t), y_t)$. The learning algorithm $f$ minimizes a slightly different notion of regret $\mc{R}^{\text{D}}_T(f)$
% % TODO here is where i'd introduce the rationale for the 2nd term.  i tihnk the real rationale is that in the absense of statistical model, we have no notion of "bayes risk", and therefore, need *somethning* to compare to.
% \begin{align*}
%     \mc{R}^{\text{D}}_T(f) &= \sum_{t=1}^T \ell(h_t(x_t), y_t) - \min_{i \in [N]} \sum_{t=1}^T \ell(h_{i, t}(x_t), y_t)\\
%     &= \sum_{t=1}^T \ell(f(h_{t-1}, x_{t-1}, y_{t-1})(x_t), y_t) - \min_{i \in [N]} \sum_{t=1}^T \ell(h_{i, t}(x_t), y_t)
% \end{align*}
% In this case, the rightmost term is the cumulative loss best out of the $N$ experts in hindsight, which depends on round $T$. There is no expectation taken over the loss, because the sequence $\mc{D}_T$ is not assumed to come from any probability distribution. If the problem is realizable, 
% % TODO gotta define "realizable", it is not obviously a definition the way you've stated it. also, not clear we need that distinction here, do we use it later?
% then one of the experts is always correct and the agent simply has to determine the all-knowing expert. Otherwise it is called unrealizable.

% % TODO i dont' understand this scenario, and in fact, i'm not sure we need either of the non-statistical scenarios in this manuscript, other than to say that they exist, and we are not talking about them here?
% In the randomized scenario, the agent submits a probability distribution $p_t = (p_{t, 1}, ..., p_{t, N})$ where $p_{t, i}$ is the weight given to expert $i$ at round $t$. That is, $f: \Delta_{N-1} \times \mc{X} \times \mc{Y} \rightarrow \Delta_{N-1}$, where $\Delta_{N-1}$ is the $N-1$-simplex. The loss incurred is weighted by the loss of each expert prediction. In this case, the learning algorithm wishes to minimize cumulative weighted loss $\mc{R}^{\text{W}}_T(f)$.
% \begin{align*}
%     \mc{R}^{\text{W}}_T(f) &= \sum_{t=1}^T \mbb{E}_{p_t}\left[\ell(h_{i, t}(x_t), y_t)\right] - \min_{i \in [N]} \sum_{t=1}^T \ell(h_{i, t}(x_t), y_t)\\
%     &= \sum_{t=1}^T \mbb{E}_{f(p_{t-1}, x_{t-1}, y_{t-1})}\left[\ell(h_{i, t}(x_t), y_t)\right] - \min_{i \in [N]} \sum_{t=1}^T \ell(h_{i, t}(x_t), y_t)\\
% \end{align*}

% \subsubsection{Reinforcement Learning}

% Another sequential learning problem, that of reinforcement learning and control, can be formalized as follows. A simple Markov decision process (MDP) is a tuple $(\cS, \cA, \{P_{sa}\}, \gamma, r)$ where $\cS$ is a set of states, $\cA$ is an action space, $P_{sa}$ is a probability measure over $\cS$ indexed by previous state $s$ and action $a$, $\gamma$ is a discount factor, and $r: \cS \times \cA \rightarrow \R$ is a reward function. When $\cS$ and $\cA$ are finite, the MDP is called a finite. 

% At time $t$, an agent operates on some policy $\pi: \cS \rightarrow \cA$ that maps a current state $S_t$ to an action $A_t$. Then, the subsequent state $S_{t+1}$ is drawn from $P_{S_t, A_t}$. 
% The goal of a policy is to maximize expected reward at time $t$, having started from state $S_0 = s$.
% \begin{align*}
%     V_{\pi}(s) = \E{}{\sum_{t=0}^{\infty} \gamma^t r(s_t, \pi(s_t)) \mid S_0 = s}
% \end{align*}
% TODO is pi here the same as h above? and  \gamma^t r(. , .) is loss? if so, can we write this explicitly as a special case of online learning?  if so, lets?  i'm fairly sure we can, and then once we do, i don't think we need to provide much of the below details in this paper.
% The expected value is taken over the sequence $S_1, S_2, ...$, where given $S_t$, $S_{t+1} \sim P_{S_t, \pi(S_t}$. The optimal policy $\pi$ depends on the true, usually unknown transition distributions $\{P_{sa}\}$. 
% % TODO why are there 'transition distributionS" (plural)? i'd have thought 1 of them is fixed a priori?
% In the case where the transition probabilities are known, the problem is called a {\it planning} problem, as no states need to be sampled for the agent to decide the optimal course of action. Remarkably, in finite MDPs, the same policy $\pi^*$ optimizes $V_{\pi}(s)$ for all choices of starting state $s \in \cS$. The optimal values $V^*(s)$ satisfy the following nonlinear system of equations
% \begin{align*}
%     V^*(s) = \max_{a \in \cA} \left\{r(s, a) + \gamma \sum_{s \in \cS}[P(s' \mid s, a)V^*(s')\right\}
% \end{align*}
% % TODO punctuate your equations everywhere please
% known as the {\it Bellman} equations. Because the optimal policy achieves this maximum, it solves
% \begin{align*}
%     V_\pi(s) = r(s, \pi(s)) + \gamma \sum_{s \in \cS}[P(s' \mid s, \pi(s))V_\pi(s')
% \end{align*}
% {\it Value iteration} and {\it policy iteration} are two canonical algorithms for solving the planning problem with theoretical guarantees. A more realistic scenario is when the transition probabilities $\{P_{sa}\}$ are not known, known as the {\it learning problem}. In this case, either the transition distributions themselves, or quantities that depend on them (such as $V_{\pi}(s)$), are estimated via actively sampling the state sequence $S_1, S_2, ...$ for training. This problem is formalized as a stochastic fixed-point problem. That is, we wish to find the vector $v \in \R^{N}$ that solves $H(v) = v$, but $H$ is inaccessible and we only have access to noisy observations $H(v_i) + w_i$ where $\E[w_i] = 0$. In this case, $N = |\cS|$, $v$ is the vector of values, $H$ is the function that represents the Bellman equation
% \begin{align*}
%     V_\pi(s) = \E{S' \mid s, \pi(s)}{r(s, \pi(s)) + \gamma V_\pi(S')}
% \end{align*}
% Given some $\alpha_t \in (0, 1)$ that governs the learning rate, updates typically look like
% \begin{align*}
%     v_{t+1} &\leftarrow (1 - \alpha_t) v_t + \alpha_t (H(v_t) + w_t)\\
%     &= v_t + \alpha_t (H(v_t) + w_t - v_t),
% \end{align*}
% which is the stochastic gradient descent update for population objective $(H(v) - v)^2$. For example, $H(v_t)$ can be approximated by sampling one state $S'$, and letting $H(v_t) + w_t$ be defined for each $s \in \cS$ by $r(s, \pi(s)) + \gamma v_t(S')$. Such algorithms can be shown to converge to the optimal policy, assuming the policy iterates $(\pi_t)_t$ visit each state and action pair $(s, a)$ an infinite number of times. Written more similarly to the supervised learning setting, we can say a learning algorithm $f_t$ at time $t$ maps the past states and actions $((S_i, A_i))_{i=0}^t$ and some additional knowledge $K_t \in \mc{K}$ (such as the past value or policy) to a new policy $\pi_t$. That is, $f_t: (\cS \times \cA)^t \times \mc{K} \rightarrow \Pi$, where $\Pi$ is the space of potential policies.

%%% ALTERNATE PROOF OF THEOREM 1

% Let $\gamma_{n_0, n_1} = \frac{R^*}{R(f(\Z'_{n_0, n_1}))}$. Take any $\epsilon > 0$, and let $E_{\epsilon}$ be the event that $\gamma_{n_0, n_1} \leq 1 - \epsilon$.
    % \begin{align*}
    %     \TE_{n_0, n_1}(f) &= \E{}{\frac{R(f(\Z_{n_1}))}{R(f(\Z'_{n_0, n_1}))}}\\
    %     &\geq \E{}{\frac{R^*}{R(f(\Z'_{n_0, n_1}))}}\\
    %     &= \E{}{\gamma_{n_0, n_1}}\\
    %     &= \E{}{\gamma_{n_0, n_1} \mid E_{\epsilon}^c}\P{}{E_{\epsilon}^c}\\ 
    %     & \quad + \E{}{\gamma_{n_0, n_1} \mid E_{\epsilon}}\P{}{E_{\epsilon}}\\
    %     &> 1 - \epsilon + \E{}{\gamma_{n_0, n_1} \mid E_{\epsilon}}\P{}{E_{\epsilon}}
    % \end{align*}
    % Because of the boundedness assumption (\ref{asm:notzero}), we have that $R(\cdot) > R_{\min} > 0$. Thus, as $n_0, n_1 \rightarrow \infty$, we have $\P{}{E_{\epsilon}} \rightarrow 0$, because
    % \begin{align*}
    %     \P{}{E_{\epsilon}} &= \P{}{\frac{R^*}{R(f(\Z'_{n_0, n_1}))} \leq 1 - \epsilon}\\
    %     &= \P{}{R(f(\Z'_{n_0, n_1})) - R^* \geq \epsilon \cdot R(f(\Z'_{n_0, n_1}))}\\
    %     &\leq \P{}{R(f(\Z'_{n_0, n_1})) - R^* \geq \epsilon \cdot R_{\min}},
    % \end{align*}
    % which goes to zero by Lemma \ref{lem:stone}. Also by the boundedness assumption, $\E{}{\gamma_{n_0, n_1} \mid E_{\epsilon}}$ is bounded from above, so $ \E{}{\gamma_{n_0, n_1} \mid E_{\epsilon}}\P{}{E_{\epsilon}} \rightarrow 0$. $\epsilon$ was arbitrary, so $\liminf_{n_0, n_1 \rightarrow \infty} \TE_{n_0, n_1}(f) \geq 1$.
    % Thus we have universal asymptotic transfer efficiency for $f$.

==> extra/framework.tex <==


\section{A Framework for In-Distribution Learning Tasks}
\label{Xapp:framework}

\subsection{An extremely brief history of machine learning theory}

\citet{Glivenko1933-wm} and~\citet{Cantelli1933-vj} wrote a pair of papers in the early 1930s that formalized learning from the perspective of probability theory.   Some 40 years later,~\citet{Vapnik1971-um} further elaborated upon these ideas.  Independent of those works (none of which were in English),  Leslie Valiant wrote a now famous article entitled, ``A Theory of the Learnable''~\cite{Valiant1984-dx}, in which he explicitly related the concept of \textit{learnable} to human learning and intelligence, following the lead of Rosenblatt, who motivated his perceptron learning algorithm similarly~\cite{Rosenblatt1958-va}. 
 All of these papers were interested in the following questions: what are the conditions under which one can use a set of data to  estimate various properties of their generative distributions. This set of papers led to the founding of statistical learning theory~\cite{Vapnik1998-po}, computational learning theory~\cite{Kearns1994-yc}, and machine learning theory~\cite{Mohri2018-tf}.   
 
 The importance of these foundational papers is profound. Since then, any machine learning task has known what its goal must be: minimize generalization error as defined in those papers.  If an algorithm could not be proved to minimize generalization error under some suitable settings, then it lacked principles and a theoretical understanding.  In other words, these papers enabled the community to distinguish between methods with strong theoretical guarantees---important for making valid statistical claims, among other reasons---and heuristics that might approximately solve some problem, but often unclear whether they do.  

Since these founding papers, however, practioners have desired to build estimators in increasingly more complex scenarios.  For example, when we have  data sampled from some distribution other than the evaluation distribution for the given task (transfer learning~\cite{Bozinovski1976-ou} or domain adaptation~\cite{Daume2007-cv}), or we have multiple tasks (multitask learning~\cite{Caruana1997-mm, Thrun1996-kk} and meta-learning~\cite{Schmidhuber1987-wy, Bengio1997-vx}), or a sequence of tasks (lifelong or continual learning~\cite{McCloskey1989-nl, Thrun1995-qy}), or more generally, what if we desire to make out-of-distribution (OOD) inferences~\cite{Bengio2011-pt}?  For each of these questions, the original ML theory formalizations are inadequate in that they make strong assumptions about the relationship between the distribution of the sampled data and the evaluation. Different OOD learning scenarios relax those assumptions in different ways, therefore requiring  new conceptual machinery to adequately characterize learning in these domains.  

Here, we restate the classical learning problem closely following standard texts~\cite{Shalev-Shwartz2014-zo, Fokoue2020-sv}.  Our departure from those works stems from our desire to generalize the formalism to allow for transfer, multitask, meta, continual, lifelong, and other out-of-distribution learning as well. The definition of learning we adopt here is informally stated in Tom Mitchell's classic definition of machine learning~\cite{tommitchell}:
% 
% \begin{quote}
    \textit{``A computer program is said to {learn} from experience E with respect to some class of tasks T and performance measure P, if its performance at tasks in T, as measured by P, improves with experience E.''}. %     -- Tom Mitchell. 
    % 1997~\cite{tommitchell}
% \end{quote}

\subsection{In-Distribution Learning Paradigms}
\label{Xapp:classic}

This subsection provides a brief informal definition of many different classic  learning  paradigms.  Each of these are characterized by having a single distribution (for training and evaluating) and a single task, though they different in terms of their goals, whether they are perceptual or active, and  batch or sequential. The implicit mentality in each of them is that the learner is learning from a blank slate, or \textit{tabula rasa}.  Perhaps this is partially because the blank slate mentality was the prevailing view in cognitive science for centuries~\cite{Pinker2003-sh}, up to and including the  the founding of artificial intelligence~\cite{McCarthy1955-kn} which was a precursor to much of learning theory.


% We first review common tasks from  classical  machine learning, to be used as running examples. The notation and ideas presented in this section will be placed into the more general framework introduced in Section \ref{sec:framework}, which is amenable to extensions such as transfer and multitask learning.
% 
% The following problems in basic statistics and machine learning are well-studied and have a strong theoretical foundation accompanied by  provably successful learners. Below we provide brief informal descriptions of various tasks with examples; in Section~\ref{sec:framework} we provide formal definitions.

\begin{description}
\vspace{2mm}
\item[Point Estimation] Given a batch of data, we assume it was generated from some distribution $P$ with parameters $\mb{\theta}=(\theta_1,\theta_2,\ldots, \theta_p)$, and we would like to estimate (possibly a subset of) those parameters. For example, we might want to estimate the likelihood of a person contracting COVID.  
% Ronak: what does complete mean here?
% JV: clarified?
\item[Hypothesis Testing] Given a batch of data, we propose a null hypothesis that the data was generated by some distribution in a null set, $P \in \mc{P}_0$, and test whether the evidence is sufficiently strong to reject this null set in favor of an alternate set, $\mc{P}_A$.  For example, we might want to test whether COVID is more serious than the flu.
\item[Supervised Learning] Given a batch of data, where each sample is a pair containing a pattern and a label for that pattern, we assume it was generated from some distribution, our goal is to find a rule such that given a new pattern without a label, we can accurately estimate the true label. In general, labels can be categorical (classification), continuous (regression), or more complicated structures (rank, networks, etc.).  For example, healthcare workers screening patients may desire to build a rule based on symptoms and exposure to estimate whether a new patient has contracted COVID. 
\item[Unsupervised Learning] Given a batch of data, where now each sample is simply a pattern, and we assume it was generated from some distribution, our goal is to find a rule that correctly assigns a label to all the patterns.  If those labels are continuous and multi-valued, 
% TODO@EE what do you mean here by multi-valued?
we are in a dimensionality reduction setting; if they are categorical, we are in a clustering setting. For example,  we may want to determine whether there are multiple clusters of COVID disease trajectories, such as `regular' COVID and `long' COVID. 
% \item[Causal Learning] Our goal in causal inference is to design experimental or observational studies such that given a batch of data including treatments, outcomes, and covariates, we can ascertain how the treatment variables are associated with the outcome variables conditional on the appropriate subset covariates. For example, we may want to determine whether a particular drug decreases the probability of mortality in COVID patients, conditional on their health~\cite{Hernan2011-yk}.
\item[Streaming Learning] Streaming learning can be any of the above scenarios with one modification: rather than estimating the quantity of interest all at once, we sequentially estimate it based on subsets of the data.  This could be because the data are arriving incrementally and/or because we have computational constraints or costs. 
\item[Online Learning] Online learning is similar to streaming learning in that we estimate the desired quantities sequentially.  The difference between online learning and the previously discussed scenarios is that in online learning, we do not assume the data were generated from one fixed distribution, but rather, that distribution may be changing in time (i.e., non-stationary), potentially even adversarially~\cite{Cesa-Bianchi2006-tv,Shalev-Shwartz2011-yd}.
\item[Reinforcement Learning] Reinforcement learning is similar to online learning, except  in reinforcement learning although we sequentially get input, we only take actions and get feedback sometimes.  This therefore introduces the need to solve a temporal credit assignment problem~\cite{Sutton2018-gx}.  
% \comE{RL is a very different animal, and would need much more detail to characterize it correctly.}
% EE please add them?
\end{description}
% TODO@JV add active learning

\subsection{Out-of-Distribution Learning Paradigms}
\label{Xapp:mtl_review}

% The following paradigms, while increasingly important in practice, generally lack an established theoretical framework that connects transfer, multitask, meta, continual, and lifelong learning together, and that shows the relationship between them and the classical learning paradigm.  By establishing a unified framework, we hope to be able to translate ideas, theorems, and algorithms across currently somewhat disconnected sub-disciplines.  Moreover, we will be able to relate these different forms of machine learning more directly to biological learning, which we argue here, is best characterized as a lifelong learning situation. 

The below out-of-distribution learning paradigms are all more complicated paradigms than the above in-distribution learning paradigms, and they are also were described more recently. Most of the in-distribution learning paradigms were described about a century ago, but many of the below paradigms are only a few decades old.  The two key differences between the above and the below are that below,  (i) the training data distribution includes data sampled from a distribution that is \textit{not} the assumed evaluation data distribution, and (ii) there may be multiple training datasets and/or tasks. 
% Perhaps it is for these reasons that they are much less studied biologically. This is despite the fact that the prevailing view in cognitive science now is that animals are born with intuitive physics, psychology, and many other relevant inductive biases~\cite{Lake2017-ip}, and that we sequentially learn more complicated concepts by leveraging prior experiences~\cite{Spelke2007-wd, Gopnik2009-zk}.  

% TODO@JV fix up

\begin{description}
\vspace{2mm}
\item[Transfer Learning] Transfer learning is characterized by their being some source information (which could be data samples, but also could be trained models, etc.), and target data associated with target task, and the goal is to leverage the out-of-distribution source data to improve performance on the target task~\cite{Pratt1993-yn, Pan2010-bv,Baxter2000-wv,Ben-David2003-fr,Mahmud2008-lp,Hassan_Mahmud2009-bd, kpotufe, Finn2017-fi, jordan2020,  Ben-David2008-tv, Dwivedi2019-hw, Shui2019-tb, Helm2020-iv}.   
% \comE{Not necessarily, and this is the issue with separating IDD vs ODD without a precise characterization of the distributional space. If the source and target distributions overlap, the goal of instance-based transfer learning is to then pick out the source data that is still in distribution, while possibly adapting those data that aren't.}
% EE I think its ok, but let's discuss
% Transfer learning is fundamental to biological learning, and has been observed even in insects with only $\approx 1$ million neurons~\cite{Giurfa2001-nr}.
% 
\item[Multitask Learning] Multitask learning generalizes transfer learning, because now there are multiple target tasks, and each dataset can simultaneously be out-of-distribution source data for some tasks, and in-distribution target data for other tasks~\cite{Caruana1997-mm,Baxter2000-wv, Jebara2011-rm, Maurer2016-qv}. In multitask learning, the learner has access to all tasks simultaneously. 
% Neuroscientists are recently starting to study multitask learning~\cite{Meyer1997-nj,Yang2019-ra,Tomov2021-rv}.   
% 
% Ronak: The multitask learning to meta-learning generalization is quite unclear to me.
% JV: better?
\item[Meta-Learning] Meta-learning generalizes multitask learning. Here, we have multiple datasets and tasks we have already trained on (like multitask learning), and now we get new queries from a new task (unlike multitask learning), and we desire to transfer from the set of previous tasks to this new task~\cite{Finn2017-fi, Cheng2019-cz, Javed2019-ck, Achille2019-it, Bengio2019-vk, Wang2020-dy, He2020, Tripuraneni2020-ab}.  
% Meta-learning has been explicitly studied in biological learning for over 70 years~\cite{Harlow1949-px}, and has recently a renewed interest~\cite{Wang2020-dy}.
% Ronak: Would it be worth mentioning something like "learning algorithms that exhibit forward transfer but catastrophically forget are meta learners, but not continual learners"?
% JV: added, ok?
\item[Continual Learning] Continual learning generalizes meta-learning, in that now there is a stream of potentially repeating tasks, and we desire to leverage previous task data to improve performance on future tasks, and also leverage current task data to improve performance on previously occurring tasks~\cite{Thrun1995-qy, Thrun1996-kk, Thrun1998-ze, Ring1997-ar, Ruvolo2013-hk, Ruvolo2013-nu, Balcan2015-ao, Pentina2014-hl,Pentina2015-xx, Finn2019-yv, Parisi2018Continual, DeLange2019Continual, Chen2018Lifelong}.  In contrast to meta-learning which focuses purely on forward transfer, the key challenge in continual learning is to avoid catastrophic forgetting and interference~\cite{McCloskey1989-nl}.
% , phenomena that have been studied somewhat in biological learning~\cite{Flesch2018-vt}, by enabling backward transfer.
\item[Lifelong Learning] Although the machine learning literature largely considers continual learning and lifelong learning to be two names for the same setting, we here view lifelong learning in a broader prospective that draws inspiration from biological learning. Consequently, we view lifelong learning as generalizing continual learning by enabling the importance of each task and computational constraints to change over the lifetime of the agent. 
% It is well established that biological agents have different priorities and resource constraints over their lifetimes to which they must adapt~\cite{Bandeira2009-js,Flood1988-ua} . 
\end{description}




\subsection{Formalization of in-distribution learning paradigms}
\label{Xapp:formal}

This section introduces learning theory largely following~\citet{Shalev-Shwartz2010} and~\citet{Fokoue2020-sv}, departing as appropriate to enable generalization in subsequent sections. %We take care throughout to consider that we will want to eventually apply this learning formalism to both machine and biological learning agents. 

\paragraph{Notation} We use the following notational conventions unless otherwise specified. Spaces of elements will be an uppercase script letter (such as $\mc{X}$ or  $\mc{Y}$). An uppercase letter (regular, unbolded) represents a single random variable (such as $X$ or $Y$). A lowercase letter represents an observation of a random variable (such as $x$ or $y$). Bold indicates a set, sequence, vector, or matrix, as appropriate (such as $\X_n$). 
% A bold uppercase letter represents a set or sequence of random variables (such as $\X_n$). A bold lowercase letter represents a set or sequence of observations of random variables (such as $\mathbf{x}_n$).
% 
The subscript $n$ on $\X_n$  represents the size/length/cardinality of the set/sequence/vector/matrix. 
% So tying together the various notations, $\X_n \subseteq \mc{X}^n$ for example can be a set of $n$-random variables $X_1, X_2, \dots, X_n$ all observed in $\mc{X}$, and we denote the set of observations as $\mathbf{x}_n$, with individual observations $x_1, x_2, \dots, x_n$. 
In an abuse of terminology, we will refer to both $\mb{X}_n$ and $\mb{x}_n$ as a dataset. And we let $[n]=\{1,\ldots, n\}$. Let $\mbb{N}$ and $\Real$ denote the integers and reals, respectively, and $\Real^d$ is $d$-dimensional reals, and $\Real_{\geq 0}$ is the non-negative reals.

We will also often refer to parameters throughout this work. In different contexts, a parameter can mean different things. When speaking about a distribution $P$, a parameter is a feature of the distribution $\theta = \nu(P)$ given by the map $\nu: \mc{P} \to \Theta$, where $\mc{P}$ is a space of distributions and $\Theta$ is a parameter space \cite{bickel-doksum}. For example, $\mc{P}$ could be Poisson, $\Theta$ could be $\mathbb{R}_{> 0}$, and $\nu$ simply gives us the rate of the given Poisson. Hence if $P = \text{Poisson}(\lambda)$, then $\nu(P) = \lambda$. We will often want to estimate these distribution parameters, and we will denote these estimators by putting a hat on the parameter of interest. Thus if we would like to estimate a parameter $\theta$, then we will generally denote its estimator by $\hat{\theta}$.
% 
We  adopt this notation in general for estimators, not just for parameters. That is, when we would like to estimate a certain quantity $\phi$, we will denote its estimator by $\hat{\phi}$. Note that as these estimators  depend on data, they are a function of it, and therefore  also random variables. 
% 
Let $\mbb{E}$ and $\mbb{P}$ denote the expectation and probability of a random variable, respectively.   
% 
% If we have then an estimator $\hat{\theta}$ for a distribution parameter $\theta$, we can inquire about the expected squared error $\mathbb{E}[(\theta - \hat{\theta})^2]$ if $\theta \in \mathbb{R}$. If the dataset with which the estimator $\hat{\theta}$ is calculated is $\X_n$, then the expectation here is taken over the distribution $P$ of $\X_n$. 
It is often assumed that each random variable is sampled identically and independently (iid) from some true but unknown distribution. 

% Ronak: I would prefer that we don't deal with the random variable versus observation technicality at all, unless it is convincingly important. Random variable notation for everything should be fine, right? Additionally, I would define v(P) = E_{X \sim P}[X], or something that is purely a function of the distribution.
% JV: why do you want to distinguish between rv and observation? that does not seem like a technicality at all to me.  observations are real data, RV's are objects that we simply assume to exist. 
% JV: i don't understand you comment about v(P), but feel free to change it as you see fit.

\subsection{The Decision Problem}

Learning problems, as will be shown below, leverage data to solve decision problems.  We therefore first formalize decision problems. Note that decision problems, as described here, do not include any data, rather, they are simply mathematical formalizations of a goal, which we will then be able to leverage to evaluate learning algorithms. The following is largely based on~\cite{bickel-doksum} (Chapter 1.3). 

 \paragraph{Query space} $\cX$. This is the space of questions, inputs, or test examples given to the agent, $x \in \cX$. While $\cX$ is often $d$-dimensional Euclidean space  more generally, it can be networks, images, text, speech, etc. 
    %
\paragraph{Action space} $\mc{Y}$.  The action space $\mc{Y}$ is the set of potential action to be returned given a query $x \in \cX$. Actions are sometimes called labels or predictions, specifically in decision problems that are \textit{perceptual}, e.g., what do we think is the answer to a given query.  In causal inference, control theory, and reinforcement learning, however, actions can be executable actions, e.g., turn left.  A few concrete examples:
\begin{itemize}
    \item Estimation: If we are estimating a real scalar-valued parameter, the action space $\mc{Y} = \Theta = \Real$.
    \item Testing: If we are testing, only two actions are under consideration: reject the null, or fail to reject the null. 
    \item Ranking: Ranking problems assign an integer to each of the data samples.  So, if there are three data samples, the action space is $\mc{Y}=\{(1,2,3), (1,3,2), (2,1,3), (2,3,1), (3,1,2), (3,2,1)\}$.
    \item Regression: If we are trying to estimate the continuous label associated with new data points, then the action space is again simply $\Real$.
\end{itemize}
Note that the action space and query space are tightly coupled.

    \paragraph{Hypothesis Space} $\cH \subseteq \{ h \mid h : \mc{X} \mapsto \mc{Y}\}$. A set of hypothesis functions that an agent considers, which is a (potentially strict) subset of all possible functions mapping $\mc{X}$ to $\mc{Y}$. Hypotheses $h \in \mc{H}$ map queries to predictions of their corresponding action. In statistics, the hypotheses are often referred to as \textit{decision rules}, and in reinforcement learning they are often referred to as \textit{policies}. A simple example of a hypothesis class is the set of linear functions~\cite{Kearns1994-yc}. 
    % Ronak: I've come upon $\mc{H} \subseteq \mc{Y}^{\mc{X}}$ and I think it's beautiful.
    % \comE{Link to choosing a learning algo + classic COLT framework}
    %
    \paragraph{Distribution} $P = P_{X,Y}$. We assume that the query-action pairs, $(x,y)$ are realizations of query- and action-valued random variables, $(X,Y)$, which are drawn from some distribution $P=P_{X,Y}$ which is an element of a set of possible distributions $\mc{P} = \mc{P}_{X,Y}$. 
    % The queries and corresponding actions are allowed to be random, and are drawn from some distribution $P_{X, Y}$ over the random tuple $(X, Y)$. 
    % Note that both $X$ and $Y$ are random variables here, unlike the classical assumption in regression (in which $X$ is a design matrix rather than a random variable), and rather than the classic assumption in machine learning (in which $X$ is a random variable, and then there exists a deterministic label function for each observed $x$).  The set \comE{Shouldn't this be bold not mc according to the notation?} $\mc{P}_{X, Y}$ is a set of distributions of random variables observed in $\mc{X}\times\mc{Y}$. \comE{I assume you mean that $X \sim \mc{X}$ and $Y \sim \mc{Y}$.  If so this, should be stated explicitly.} 
    For technical reasons, we require that each distribution $P \in \mc{P}$ 
    % \comE{Bold since it is a set?} 
    has positive probability over the full query and action space, that is, $\mathrm{supp}(P)=(\mc{X},\mc{Y}), \, \forall P \in \mc{P}$.
    % Ronak: What technical reasons?
    % JV: because otherwise it is silly to assert that \mc{X} is \mc{X}, if one can *never* sample a query from some part of it, right?
    \paragraph{Risk} $R : \mc{H} \times \mc{P} \mapsto \R_{\geq 0}$. A risk function takes a hypothesis and a distribution on the random variable $(X, Y)$ and evaluates the performance of that hypothesis against the distribution. We typically think of $R$ being parametrized by $P_{X, Y}$, and taking only a hypothesis $h$ as its single argument.
Often, implicit in the risk functional, is a loss function $\ell: \mc{Y} \times \mc{Y} \mapsto \mbb{R}_{\geq 0}$, and the risk is defined as the expected loss with respect to $P_{X, Y}$ 
\begin{align*}
    R_P(h) = \mbb{E}_{X, Y}[\ell(h(X), Y)] = \int_{\cX,\cY} \ell(h(X), Y) dP_{X,Y} \enspace.
\end{align*}
More generally, risk can be any arbitrary functional of the loss, including the median for example. 
% such as $\P{X, Y}{\ell(h(X), Y) \geq 0.1}$.  \comE{Unclear.}
% 
Risk need not be defined in terms of loss, rather, risk can explicitly be a function of the distribution and hypothesis directly. 




Aside from the distribution, $P_{X,Y}$, the above mathematical objects are typically provided in the specification of a problem.  Hereafter, we refer to the source of these objects as the `Boss'. 
% the so-called ``Boss" , because they are typically specified \textit{a priori}. 
% \comE{``ML Engineer''?} % TODO@jovo discuss with eric
On the other hand, the true distribution governing the queries and actions, $P_{X, Y}$, is not chosen by the Boss, but rather, chosen by ``Nature''.  If the true distribution is known, the decision problem is relatively straightforward.  Given these components, we can define a {\bf decision problem}:

\begin{definition}[Decision Problem]
    A \textit{decision problem} has the form 
    \begin{equation} \label{XAeq:problemA}
    \begin{array}{ll}         
         \textnormal{minimize}  &R_P(h) 
        %  \mbox{\comE{Doens't this require $\mc{P}_{X,Y}$, or are you assuming it is implicit in $R$?}}
        \\ \textnormal{subject to }\,  &h \in \cH
    \end{array} \enspace .
    \end{equation}
\end{definition}
Let $h^\diamond$ denote a \textbf{class optimal hypothesis} that minimizes Equation~\ref{eq:problem}, and let $R^\diamond = R(h^\diamond)$ denote the \textbf{class optimal risk}.  Note that $h^\diamond$ need not be unique, and in fact, it need not even exist (in which case we could be looking for an infimum rather than a minimum).
Moreover, whenever $\cH$ is a strict subset of all possible mappings from $\cX$ to $\cY$, the optimal risk for a given decision problem may not be the minimal risk achievable by any possible hypothesis.  Let $R^*$ denote the \textbf{Bayes optimal risk} for a given decision problem without the constraint that $h \in \cH$, and $h^*$ denote a \textbf{Bayes optimal hypothesis} that achieves $R^*$ (which again, in general, need not exist nor be unique). 
% relaxing \comE{what do you mean by relaxing?} the specified $\cH$ to . 
Given this definition, we can define the \textbf{excess risk} or \textbf{model error} as $R^\diamond-R^*$ ~\cite{Vapnik1998-po}.  Figure~\ref{fig:schematic}(A) illustrates the various components and which players contribute which components of a decision problem. 




\subsection{The Learning Problem}
\label{Xapp:task}

Solving decision problems depends on knowing the true distribution, $P_{X,Y}$. In learning problems, the true distribution is  partially or completely unknown, and so, a learner must leverage data to estimate hypotheses.  A {\bf learner} uses $n$ data points to provide a good guess for $h$ in the sense of Eq.~\eqref{eq:problem}. This is the learning task. Defining it formally requires a few additional concepts.
% \begin{itemize}
    % \item 
    \paragraph{Data Space} ${\mc{S}^*}$. Let $s \in \mc{S}$ denote a data sample. Data samples can be query-action pairs in supervised learning problems, that is, $\mc{S} = \mc{X} \times \mc{Y}$, however, more generally, they need not be (for example, consider unsupervised learning in which case samples might purely be in $\mc{X}$). 
    % or in a problem like mean estimation of a Gaussian, observations from that Gaussian.  
    We desire learners that can operate on any sample size.
    For example, consider the  \texttt{randomForest.fit()} as a mathematical function: it can operate on $n$ query-action pairs, $\{(x_i,y_i)\}_{i \in [n]}$, for any $n$.  Thus, the input space for \texttt{randomForest.fit()} must enable various sample sizes.
    Moreover, in natural language processing settings, the input is frequently sequences of words of different lengths.  
    Because of this, let $\mc{S}_0, \mc{S}_1, \mc{S}_2, \ldots$ be a sequence of data spaces with fixed sample sizes of $0, 1, 2,\ldots$ data samples per space.   
    Our data space is the union on this sequence, that is,  ${\mc{S}^*} = \bigcup_{n = 0}^{\infty} \mc{S}^n$. 
    % \comE{Not clear why $\bigcup_{n = 0}^{\infty} \mc{S}^n$? Because n is a variable?} 
    Thus, $\mc{S}^*$  is the set of all $n$-length lists of $\mc{S}$-valued data, for any $n$. 
    % The $n = 0$ case, $\mc{S}^0$, here implies the empty set, $\varnothing$, meaning no data.  
    % Note that in many supervised learning problems, the data space is defined by the product of the query and action spaces, that is, $\mc{S}= \cX \times \cY$, but this is just a special case of considerable interest. 
    % \item 
    
\paragraph{Statistical Model} $\cP=\cP_{\D,X,Y}$, is a collection of distributions. Recall from the definition of a decision problem, we assumed that query-action pairs were sampled according to some distribution $P_{X,Y} \in \mc{P}_{X,Y}$.  In decision problems, the query-action distribution was known, and therefore, hypotheses could be evaluated with respect to the true distribution.  In learning problems, the query-action distribution is unknown, and therefore, a learner (defined below) leverages data to obtain a good approximate hypothesis.  We assume that a training dataset, $\mb{s}_n=\{s_1, \ldots, s_n\} \in \mc{S}^n$, is sampled  from 
    % $P_{X,Y}$ as well, though sometimes only $X$ is observed. 
some training dataset distribution $P_{\D_n}$, which is an element of $\mc{P}_{\D_n}$, and $\mc{P}_{\D} = \cup_n \mc{P}_{\D_n}$. \textbf{For in-distribution problems, there is a strong (often implicit) assumption on the relationship between each $P_{\D_n}$ and $P_{X,Y}$: specifically, it is assumed that the queries are about $P_{\D_n}$, that is, queries are about the distribution that we assume the training data are sampled from.} For example, in hypothesis testing, we query whether the data distribution is in the null or alternative model (even if the true data generating distribution is in neither). In estimation, we query about the parameters of the assumed generative model (e.g., the mean of a Gaussian, even if the true data generating distribution has fat tails). In supervised learning, we may query about what is the most likely label for a particular pattern, again under the in-distribution assumption.  
Commonly, it is assumed that each training observation is sampled independently and identically  (iid) from the same fixed  query-action distribution, that is, $P_{\D_n} =\prod_{i \in [n]} P_S$. Moreover, in supervised learning, it is commonly assumed that   $P_S = P_{X,Y}$. 
    % though this assumption can be relaxed for certain in-distribution learning problems (such as online learning).
    % , in which case we have that $P_{\D_n}=\prod_{i \in [n]} P_S$.
    % The full  distribution for a given learning problem therefore is the joint distribution of the training dataset, and the joint distribution of the query-action pairs.
    % 
    Note that whether or not we have an in-distribution learning problem, the true but at least partially unknown joint distribution $P_{S,X,Y}$ need not be an element of the model $\mc{P}_{S,X,Y}$, which is simply the set of distributions that the Boss has decided (for some reason) to focus on.  

    % \textbf{The key departure of our learning problem set up, from those defined in the standard textbooks, is that $P_S$ and $P_{X,Y}$ can be different. } When the two are different, we have an out-of-distribution learning problem, and when they are the same, we have an in-distribution learning problem. We will leverage this difference to define Mitchell Learnability and learning efficiency, which quantify whether and how much a learner learns, respectively. 
    
    
    \paragraph{Learners} $\mc{F} \subseteq \{f: \mc{S}^* \times \Lambda \} \mapsto \cH'$,  where $f$ is a learner, and $\cH'$ is the set of hypotheses that $f$ can yield. Note that in general, $\cH'$---the set of hypotheses that $f$ can find---and $\cH$---the set of hypotheses that are allowed by the decision problem---need not be the same.  For example, the decision problem may be looking for any linear function, but the learner we use may only search over linear functions of the form $h(\mb{x})= \mb{x}\T \mb{\Sigma}^{-1} \mb{\delta}$, i.e., linear discriminant analysis. 
    % 
    The first input to the learner is the data which the learner will utilize to learn a hypothesis, $\mb{s}_n \in \mc{S}^*$. The second input is the hyperparameter, $\lambda \in \Lambda$, which can  incorporate prior knowledge, initial conditions, or any other hyperparameters for the learner. 
    % 
We will typically suppress the $\Lambda$-valued inputs for notational brevity.  
% \comE{What is $\cH'$?}


    % \item 
    \paragraph{Error} $\mc{E}: \mc{F} \times \mc{S}^* \times \mc{P} \times \mc{R} \mapsto \Real$, where $\cR$ is the set of possible risk functions.   Because the error of the learner depends on the data, which we assume are realizations of random variables, the risk is also a random variable. The error measure is therefore always some function of this random variable.  
For example, it is common in statistics to seek learners with small \textbf{expected risk} (also called {\bf generalization error}). Letting $\hat{h}_n=f(\D_n)$ be the model learned from dataset $\D_n$ by learner $f$, the expected risk  of $\hat{h}_n$
% of $f$ applied to different datasets?} 
is given by
\begin{equation} \label{XAeq:excessriskA}
    \mbb{E}_{\D_n \iid P} [R(\hat{h}_n)] = \int_{\cS^n} R(f(\D_n)) dP \enspace .
\end{equation}

\noindent 
When risk is defined as expected loss, the above equation can be further expanded as follows

\begin{equation}
    \mbb{E}_{\D_n \sim P_{\D_n}} [\mbb{E}_{P_{X,Y}} [\ell (f(\D_n)(X),Y)]] = \int_{\cS^n}  \int_{\cX,\cY} \ell(f(\D_n)(X), Y) dP_{X,Y} dP_{\D_n}
    \enspace , % = \mbb{E} [\hat{h}_n],
\end{equation}

\noindent 
where the internal integral is over query-action pairs $(X,Y)$, and the external integral is over datasets $\D_n$.
Equivalently, one may desire to minimize the \textbf{expected excess risk} of $\hat{h}_n$ relative to $R'$, which could correspond to { the class optimal risk} $R^\diamond$ or {the Bayes optimal risk} $R^*$, 
% TODO@ali see comment below
% ali to jovo, yup makes sense 100$. duly noted for the future.
% \comE{Ali -- note that anywhere you reuse notation from a while ago, you should assume that the reader won't remember it and so should add in text descriptions, as I've done here}
\begin{align} \label{XAeq:pacA}
    % \E{}{R(f(\D_n))} - R^* =   
    \mbb{E}[R(\hat{h}_n)] - R' \enspace,
\end{align}
where we dropped the subscript on $\mbb{E}$ for brevity. 
In machine learning, it is common to instead be concerned about finding hypotheses that achieve relatively low excess risk with relatively high probability. 
% Let $\eps_n$ be a monotonically decreasing function of $n$, and let $\delta >0$ be some positive constant.  Now we search for hypotheses that are probably approximately correct:
% \begin{align} \label{XAeq:online}
    % \mbb{P}\left[ R(\hat{h}_n)) - R' \leq \eps_n \right] \geq 1-\delta.
% \end{align}
In other cases, we might care about minimizing the worst that our learned hypothesis could be expected to perform over a set of possible different unknown distributions $P$, the so-called \textbf{minimax} solution.
% 
% Note that above, the estimated hypothesis $\hat{h}_n$ can be changing with each sample, whereas in the above definitions, we compare a fixed hypothesis $\hat{h}_n$ with some alternative.  \comE{Confusing... two references to "above"}
We define \textbf{error}, $\mc{E}_f(\D_n)$ of a learner $f$ on dataset $\D_n$  as being any one of 
% the above equations,
Equations~\eqref{eq:excessrisk}--\eqref{eq:pac},
 or  related variants.  
%  Note that the above equations could equally well have been written in terms of $f(\D_n)$ rather than $\hat{h}_n$. 
We have implicitly assumed in this discussion that our learner $f$ is not a randomized algorithm, rather, it is a deterministic function of its input $\D_n$.  The above could all be generalized to include, for example, an expectation over the randomization of $f$ if one desired to explicitly study random algorithms, but we do not address them further here.  

% \end{itemize}






% \comE{Lacking a macro view of where you're heading at this point.} 


% 
Combining all of the introduced components, we can now define an  {\bf in-distribution learning task}.  The learning task is often defined in terms of a \textit{specific} learner $f$, that is, the task of the learner is to find a hypothesis $h$ with small error.  This definition of a task makes sense from the perspective of classical learning theory, in which we desire to understand the properties of a given $f$.  Moreover, from the perspective of biological learning, an agent (and specifically, its brain) may implement a given learner $f$. Nonetheless, we define a learning task with respect to a set of possible learners $\cF$, because this corresponds to machine learning practice, in which we search over $\cF$ for one that performs the `best' according to some suitable notion of performance. 
% 


\begin{definition}[Learning Task] \label{XAdef:task}
    Given a query space $\cX$, action space $\cY$, hypothesis class $\cH$, risk function $R$, and $n$ samples $\D_n$ drawn according to some true but unknown  distribution $P$,  the task $t$ is to choose an $f \in \mc{F}$ that learns a hypothesis $\hat{h}_n$
    that minimizes  error $\mc{E}$  by learning from $\D_n$:
    \begin{equation} \label{XAeq:task}
    \begin{array}{ll}         
         \textnormal{minimize}  & \mathcal{E}_f(\D_n) \\ 
        \textnormal{subject to }\qquad  &f \in \cF
    \end{array} \enspace .
    \end{equation}
\end{definition}
% 

Note that the clause ``learning from $\D_n$'' is not explicitly incorporated into Equation~\eqref{eq:task}, in that it is conceivably possible to minimize error without using $\D_n$ at all (for example, imagine $f$ always outputs an $\hat{h}$ that predicts class 1; for tasks where such hypotheses are optimal, $f$ will have minimized error, but not by using data).  We will return to address this limitation of the above definition later. 
We think of a learning task as having three different players.  The Boss, as previously mentioned, also provides the data space $\cS^*$, statistical model, $\cP$, learner space $\cF$,  and error $\cE$.   Nature provides the true distribution, $P_{S,X,Y}$, which includes a distribution over queries which are about the assumed distribution governing the data.
% , which now includes a distribution over the data. 
% \comE{Add in the notation for each of these elements.}  
The third player in this game, the machine learning practitioner, gets to choose an $f$ on the basis of theoretical understanding, empirical performance, and domain specific knowledge. Figure~\ref{fig:schematic}(B) illustrates the various components and which players contribute which components of a learning problem. 
% \comE{General comment.  You might consider using notation of the nature-given $P$ and the estimated/chosen $\hat{P}$ instead.} 



\paragraph{The value of a formal task definition} Often in machine learning a given $h$ is only appropriate for one of the learning scenarios defined in Section~\ref{sec:classic},  and a given $f$ only learns for one of those scenarios as well.   However, in general, we often want $h$'s to be more general, to be able useful for many different kinds of scenarios, and we want $f$'s to be able to learn $h$'s that are appropriate for those scenarios.  For example, given some data, we might want  to be able to learn to classify points, identify which features are important, answer questions, etc. 
% Indeed, in biological learning, sometimes agents receive true labels (in which case they are performing supervised learning) and sometimes they get no external feedback whatsoever (in which case they are performing unsupervised learning).  
In Sections~\ref{sec:framework} and later, we will begin introducing learners $f$ that can flexibly adapt as different components of the learning task change.
% \comE{Sorry, but I'm not following this paragraph. Wouldn't the problem be the choice of learners $\cF$?}
% EE: i tried to fix.

% \comE{ERIC STOPPED EDITING HERE.}




\paragraph{Learners vs. Hypotheses}
% 
In learning problems, the Boss specifies the data space, assumed data model, and learner class, in addition to the decision problem. In general, the Boss can define the hypothesis and learner sets independently, and often does so.  In such scenarios, it may be the case that the domain of the hypothesis set $\cH$ is not equal to the co-domain of the learner set $\cH'$.  If it happens to be the case that the intersection of these two sets is empty, $\cH' \cup \cH = \varnothing$, then the Boss has failed to specify a learning problem with a viable solution.  However, as long as their intersection is non-empty, one can minimize the objective defined  in Eq.~\eqref{eq:task}. 


When their intersection is non-empty, but also non-equal, it may be the case that $f$ outputs an element of $\cH'$ that is not in $\cH$.  In such settings, 
one can define a (projection) map  from the co-domain of $f$ to the domain of $h$  to get a valid hypothesis. For example, if $\mc{H}$ is linear functions only, and $f$ outputs quadratic hypotheses, then the projection map could be simply dropping the quadratic term and keeping only the linear term. Formally doing so requires redefining $\cH'$ to include this projection operation. 

Note that the distinction between learners and hypotheses is often ambiguous in notation and definitions.  For example, there are two quite different random forest functions, both colloquially called `random forest'.  \texttt{RandomForest.fit} is a \textit{learner} $f$, so it takes as input a dataset, $\D_n$, and some hyperparameters (e.g., specifying the number of trees, etc.). The output of  \texttt{RandomForest.fit} is the \textit{hypothesis} $\hat{h}_n=$\texttt{RandomForest.predict}, which takes as input a single query $x \in \cX$, and outputs a single action $y \in \cY$. 
% 
For simplicity of presentation, in the sequel we will assume that the co-domain of all learners $f \in \cF$ coincides with $\mc{H}$.


\paragraph{Computational complexity}
% 
So far, we have not explicitly mentioned computational complexity (in classical statistical estimation and hypothesis testing, and decision theory, it is rarely discussed)~\cite{Van_Rooij2019-hu}. In the context of a learning task, we consider both space and time complexity for both the learner $f$ and the learned hypothesis $\hat{h}_n$.  Because there is no strict requirement that any given computation happens at the learner or the learned hypothesis,  we often make the standard assumption that any bounds we place on $f$ are also placed on $\hat{h}_n$. Moreover, because space complexity lower bounds time complexity, and we are only concerned with upper bounds here, we can restrict further discussion to time complexity of $f$. And therefore, we can refer to the \textit{resources} required for a given learning problem to refer to the computation time of $f$, which in turn bounds computational space of $f$, and both space and time of $\hat{h}_n$.  That said, $\mc{F}$ and $\mc{H}$, both provided to us by the Boss, might include both space and time complexities.  
We will use both \textit{Big-O} and \textit{little-o} notation. 
Specifically, we write $f(x) = \mc{O}(g(x))$ as $x \rightarrow \infty$ if $f$ is at most a positive constant multiple of $g$ for sufficiently large values of $M$; that is, 
$f(x) = \mc{O}(g(x))$ if there exists a positive real number  $M > 0$, and a real number   $x_0 \in \Real$ such that  $|f(x)| \leq M g(x) \, \forall x \geq x_0.$ 
% 
And we write $f(x) = o(g(x))$ as $x \rightarrow \infty$ if for every positive constant $\eps$ there exists a constant $N$ such that
% 
$|f(x)| \leq \eps g(x)\, \forall \, x \geq N.$ Computational complexity considerations will be particularly important in sequential decision making and learning scenarios, which we discuss below.


% 
% With the above definitions, the definitions of a learning task, and learnability, are straightforwardly generalized into this sequential learning setting, essentially by adding summands in the appropriate places. 
Appendix~\ref{app:sequential} provides some formal definitions of in-distribution sequential learning problems, and Appendix~\ref{app:def} provides formal definitions of PAC learnability, non-uniform learnability, and consistency using our notation.





==> extra/intro.tex <==
The core tenets that constitute learning have remained elusive for practitioners of artificial intelligence (AI), and the larger scientific community. A rigorous and expressive mathematical model of learning contributes not only to better intelligent systems, but to a thorough understanding of the brain.

Previous notions of learning include that of \citet{tommitchell}, in which (loosely), an agent, or learning rule, $f$ learns from data $\mc{D}$ if its performance $\mc{E}$ on task $t$ improves by virtue of seeing $\mc{D}$. The statistical pattern recognition community often casts data $\mc{D}$ as independent and identically distributed draws of input-output pairs from some distribution, say images and labels of whether or not the image contains a cat. The agent $f$ outputs some hypothesis function that maps inputs to outputs. $\mc{E}$ is an error function which can measure the expected deviation of predicted from actual outputs, for example. In this framework, the basic criterion for a learning rule is to be consistent, that is that the error of the hypothesis converges in probability to the optimal error as the amount of data increases to infinity. \cite{Devroye1997-bd} The probably approximately correct (PAC) learning framework of \citet{Valiant1984-dx} extends these ideas by studying not only whether the error converges, but the rate. \cite{Mohri2018-tf} This puts a first-order efficiency criterion on learning, beyond the zero-th order condition of consistency.

These arenas are well-studied, and have incubated the rich theory and applications of machine learning, including speech/language processing, computer vision, and autonomous vehicles. However, these paradigms do not attempt to formalize the human ability to jointly learn multiple tasks, nor do they address the aspect of learning that is sequential in task as opposed to sequential in data. Instead, they adopt the {\it tabula rasa} approach, in which learners with no prior knowledge observe some number of examples specific to a particular task, and are evaluated on that task's performance. Humans, on the other hand, learn to crawl before they can walk, and walk before they can run. Both the order of these tasks, and the transfer of knowledge between the tasks, are highly relevant components of the learning process. We seek learning systems that can perform better on current and future tasks by virtue of leveraging previous tasks, a phenomenon known as {\it forward transfer}. Even if forward transfer is achievable, learners can {\it catastrophically forget}, or decrease their performance on previous tasks after having learned the current tasks. \cite{pl} We seek to not only avoid this pitfall, but actually exhibit {\it backward transfer}, or increasing past performance by using current and future data. This setting, called {\it lifelong learning}, is a departure from previous approaches, in that good learning algorithms are to exhibit omnidirectional transfer. There are other ways of measuring lifelong performance. \citet{Benavides2018} for example defines a cumulative gain metric, which, roughly, can be a measurement of how much backward transfer each additional task induces, allowing lifelong learning rate measurement. Multiple tasks also opens questions of adversaries, or tasks that are specifically designed to induce catastrophic forgetting. 

Transfer learning, multitask learning, meta learning, and learning to learn have all explored this territory, typically in the context of algorithms in specific domains, evaluated by performance on benchmark datasets such as Split-MNIST. \cite{3scenarios} \citet{Thrun1995-qy} gives the first major treatment of the lifelong learning, places approaches into two algorithmic frameworks:
\begin{itemize}
    \item fitting models with both parameters specific to particular tasks and parameters shared across multiple tasks \cite{ruvolo2013ella}, and
    \item injecting an inductive bias that decreases the effective amount of hypothesis functions from which the agent has to choose. \cite{Finn2019-yv}. 
\end{itemize} 
Other approaches ``replay"  previously encountered data to promote forward transfer~\cite{kirkpatrick2017overcoming}. However, the definition of lifelong learning in \citet{Thrun1995-qy} is still colloquial. To our knowledge, the community has yet to establish a theoretical framework and formal criterion by which an algorithm can claim it has decidedly ``lifelong learned". We address this gap in this manuscript, by
\begin{enumerate}
    \item formulating the transfer, multitask, and lifelong learning problems in the context of statistical decision theory,
    \item proposing {\it ensembling representations} as a generic meta-algorithm to approach these problems
    \item presenting {\it ensembling partitions} has a particular instantiation of ensembling representations, based on the classical histogram rules of \citet{Devroye1997-bd}.
\end{enumerate}
We hope that this work brings multiple, formal tasks, sequential learning, and representation sharing to the forefront of the push toward achieving truly intelligent AI systems.

==> extra/learning_tasks.tex <==
\section{In-distribution learning paradigms as learning tasks}
\label{app:classic}

Classical statistics and machine learning problems can be cast into the framework of learning tasks, as defined above. We therefore restate the examples given in  Section \ref{sec:prelims} using the concepts defined in Section \ref{sec:framework}.
\begin{example}[Point Estimation]
    All point estimation problems are learning tasks  with the following properties. We have a dataset $\D_n$, and we assume it is sampled (typically iid) from $P_{\bth} \in \mc{P}$, where $\mc{P}= \{ P_{\bth} : \bth \in \bth\}$. The query space is the single query, `What is true $\theta$?'', where $\theta \subseteq \bth$ is a (possibly complete) subset of the potenitally multivariate parameter characterizing the distribution, $P_{\bth}$. The action space is $\cY = \mb{\Theta}$, as the learner will output the static estimate $f(\D_n)=\hat{\theta}$, the sample space is the set of all possible sets of realizations of the random variables $S_i \iid P_{\bth}$ for $i \in [n]$. Here,  $\cH $ the set of constant functions on $\mc{X}$ (defining $\cH$ is an overkill for point estimation). %The reset is flexible.
    % There are many commonly used choices for $R$, $\cP$, and $\cF$.  
    % 
    % For example, $R$ could be squared error $R(h) = \E{}{(h(X) - \theta)^2}$,  $\cF $ could be maximum-likelihood estimator, and $\mc{P}$ could be iid Gaussians. 
\end{example}

As a specific example, consider the problem of mean estimation for a univariate Gaussian with known variance. The query space is then $\{$"What is $\mu$"$\}$ where $\mu$ is the mean of the Gaussian. The action space is then $\mathbb{R}$. The data space is $\mc{S}^* = \bigcup_{n \in \mbb{N}}\mathbb{R}^n$ as the normal distribution is a distribution on the real line. The learner class could be a single learner, being the maximum likelihood estimator. Explicitly, 
$f(\D_n) = \big(\frac{1}{n}\sum_{i = 1}^{n}S_i\big)(\cdot) = \hat{\mu}(\cdot)$, so that $h(X) = f(\D_n)(X) = \hat{\mu}(X) = \hat{\mu}$. The risk  is  $R(h) = \mathbb{E}\left[(\hat{\mu} - \mu)^2\right]$. $\mc{P}$ could be all Gaussians with finite variance.
% TODO@ali above you said H is the set of constant functions, but here you define it to eat a single X.  here, h eats "what is theta", since that is the query, right?
% ali to jovo: yup exactly. in this case, the hypothesis space is the same size as R. for each real number x, there is a corresponding hypothesis h_x such that h_x("what is theta") = x. so technically yeah all the hypotheses are constant on the query space since there is only 1 query in the query space.

\begin{example}[Hypothesis Testing]
     Hypothesis testing problems are learning tasks with the following properties. 
     $\mc{X}$ is again a singleton set with the query being "Should the null hypothesis be rejected?". The action space is $\cY = \{0, 1\}$, denoting ``fail to reject" and ``reject" at the given significance level $\alpha$. The hypothesis class is simply a tuple: $\cH = \{H_0, H_A\}$, where $H_0 \subsetneq \mc{P}$ is a subset of distributions in a model of distributions under consideration $\mc{P}$, and $H_A$ is another non-overlapping subset, that is, $H_A \subsetneq \mc{P}$, and $H_0 \cap H_A = \varnothing$. %, where $h_t$ is identically $t$ on $\mc{X}$. 
     $R$ is the power for a specified $\alpha$-level test.  The data space is again the set of all possible sets of realizations of the random variables $S_i \iid P_{\bth}$ for $i \in [n]$.
     can be quite general,  $\mc{S}^*$, as can the model $\mc{P}$. $\cF $ is any valid learner $f$ (testing procedure), that is, learners such that $\sup_{P_0 \in \mc{P}_0} P_{0}[f(\D_n) = 1] \leq \alpha$. %$\mc{P}$ could again be Gaussians over $\mc{D}$ (again assuming iid data).
\end{example}

As a specific example, we could have the classical situation where we have a normal with unknown mean $\mu$ and known variance $\sigma^2$. The null hypothesis is $\mu = 0$, and the alternative is $\mu > 0$. $\mc{S}^* = \bigcup_{n = 1}^{\infty}\mbb{R}^n$. The query, action, hypothesis, and risk spaces are as above. The learner class could be the single learner that outputs the indicator that the likelihood ratio statistic is greater than some $C$.  Let $\ell$ be the log likelihood, $\theta_0 = 0$, and $\hat{\theta} = \sup_{\theta \in (0, \infty]}\ell(\theta; \D_n)$, then we have
\begin{align*}
    \Lambda(\D_n) & = 2\big(\ell(\hat{\theta}; \D_n) - \ell(\theta_0; \D_n)\big)(\cdot) \\
    f(\D_n) & = \mbb{I}\big(\Lambda(\D_n) \geq C\big).
\end{align*}
Let $C$ be such that 
\begin{align*}
    \mbb{P}\big(h(X) = 1\big) \leq \alpha,
\end{align*}
where $h(X) = f(\D_n)(X)$. 
% TODO@ali cross-reference with Ben Recht textbook and see if we want to revise based on anything he wrote. 
% ali to jovo: this is all in appendix, maybe dones't matter?

\begin{example}[Supervised Learning]
In supervised learning problems, each data sample is a query-action pair, $s_i=(x_i,y_i)$, so $\mc{S}=(\mc{X} \times \mc{Y})$.  We again obtain a data $\D_n$ which we assume is sampled iid from some $P \in \mc{P}$.  When $|\mc{Y}| = \infty$ it is a regression problem, and when $\mc{Y}$ is categorical, %$|y_i-y_j| \in \{0,1\} \, \forall i,j$, 
it is a classification problem. % Here, the query space is $\mc{X}$. The action space is $\mc{Y}$. $\cH$ can be all linear functions, or all functions parameterized by weights in a particular neural network architecture. $R$ can be the probability of misclassification or mean squared error. The data space $\mc{S} = \cX \times \cY$. $\cF = $ all learning learners that fit in polynomial time in $n$, for example. A distribution $P$ could be the product of a Gaussian over $\mc{X}$ and an arbitrary probability mass function over $\mc{Y}$ (if $\mc{Y}$ is countable), and then $\mc{P}$ is the set of all such distributions.
\end{example}
% TODO@ali is \mc{R} ever *not* a single risk function for a specific task? assuming it is, we should clarify that. 
% ali to jovo: this is all in appendix, maybe dones't matter?

As a specific example, the query space can be $\mc{X}$ could be $\mbb{R}^d$. The action space is $\mc{Y} = \mbb{R}$. $\mc{R}$ could be the single risk function $R(h) = \mathbb{E}\left[(h(X) - Y)^2\right]$, where $Y$ is the correct action. The learner space $\mc{F}$ could be all the learners that utilize the method of least squares but with different penalty terms (incorporated as a hyperparameter for example). Explicitly, $\hat{h}_n = f(\D_n) = (X\T X + \lambda I)^{-1}X\T y(\cdot)$, where $X$ is the $n\times d$ matrix of $\mc{X}$ queries, $y$ is the $n\times 1$ vector of corresponding correct actions, $\lambda$ is the penalty factor, and $I$ is the $n\times n$ identity. $\mc{P}$ could be multivariate Gaussians on $\mathbb{R}^d\times\mathbb{R}$ with covariance matrix $\sigma^2I$, for some $\sigma^2 > 0$, and mean zero for each component. 

\begin{example}[Unsupervised Learning]
Unsupervised learning differs from supervised learning in that $\mc{S}=\mc{X}$, that is, the data samples lack paired labels. It also differs in that sometimes $f$ learns a mapping from $\D_n \to \mc{Y}^n$, rather than a mapping from $\mc{X} \to \mc{Y}$.  For example,  many manifold learning algorithms learn low dimensional representations of the observed data, but fail to provide a mapping function to enable answering queries on new data (the ``out-of-sample embedding'' problem).  When $\mc{X} \subseteq \Real^p$ and $\mc{Y} \subseteq \Real^q$, and $p < q$, it is a dimensionality reduction problem.  When $\mc{Y}$ is categorical, 
% $|y_i - y_j| \in \{0,1\} \, \forall i,j$, 
it is a clustering problem. 
    % For unsupervised learning, both the query and data spaces can be some $\cX$. The action space $\cY =$ some representation space, such as a subspace of $\cX$ (if $\cX$ is a vector space), or a cluster assignment. $\cH$ could be projection matrices onto the subspace of $\cX$. $\mc{R}$ includes functions like the average distance to the cluster mean or the expected reconstruction error. Like before, $\cF = $ all learning learners that fit in polynomial time in $n$. Finally, $\mc{P}$ could be simply Gaussians over $\mc{X}$.
\end{example}

As a specific example, the query and data sample spaces are the same, $\cS = \cX = \mbb{R}^d$. The action space is $\cY = \{1, \dots, k\}$, where $k$ is some number of clusters in $\mbb{R}^d$. The learner class can be the single learner of K-means (where $K = k$). The hypothesis is the cluster assignment function which given a query $x \in \mbb{R}^d$ outputs which cluster (i.e. a number in $1, \dots, k$) it should correspond to. The risk could be the single function of the expected mis-assignment probability. Finally, $\mc{P}$ could be the product of multivariate Gaussians for $\mc{D} = \mc{X} = \mbb{R}^d$, and any probability mass function over $\mc{Y} = \{1, \dots, k\}$.




\section{Sequential Decision Making and Learning} 
\label{app:sequential}



In the above sections on decision and learning tasks, it was implicit that we were operating in `batch mode', that is, we obtained all the data at once, and then only had to make a single decision, and learn a  hypothesis only once.  Decision making and learning in batch mode can reasonably be thought of as special cases of a more general form of decision making and learning which we will refer to as sequential decision making and learning.  These sequential problems have been addressed in various different communities, and variants often go by the same name, adding confusion to the literature. For example, the following is a short list of the names of problems that fall under the general category of sequential decision making and learning: sequential prediction~\cite{Rakhlin2015-bi}, online learning~\cite{Shalev-Shwartz2011-yd}, forecasting and games~\cite{Cesa-Bianchi2006-tv},  system identification~\cite{Ljung1998-cf}, control theory~\cite{Boyd1994-vz}, and reinforcement learning~\cite{Sutton2018-gx}. A key to all of them, however, is that there is a specific hypothesis $h$, which is the target hypothesis to sequentially learn.  The learners may have bounded complexity, limited feedback, face an adversarial competitor, but they still have the same goal of learning a specific fixed $h$ with desirable error properties.  
% Dynamical systems problems provide classic examples of sequential decision tasks.  Sequential decision tasks, like batch decision tasks, differ from their learning counterparts insofar as the distribution governing the data is known \textit{a priori}, so the job is simply to choose the hypothesis that minimizes risk.  For example, the Kalman Filter provides an inference of the most likely latent state, given a sequence of measurements under  linear and Gaussian dynamical system assumptions.  When the distribution governing the data is unknown, the problem is classically referred to as \textbf{system identification}, or more generally, \textbf{reinforcement learning}~\cite{Hardt2021-ty}. The counterpart to Kalman Filters in the sequential learning scenario is the Baum-Welch algorithm, which can be used to jointly estimate the parameters governing the dynamical system, as well as infer the most likely latent states~\cite{Rabiner1989-mr}. 
% 
To formalize sequential decision making and learning requires modifying a few of the previously introduced concepts. We are a bit less formal in this section than the previous section for brevity and simplicity of presentation. 
% \begin{itemize}
    % \item 
    \paragraph{Statistical Model} $\cP_{S,X,Y}$. The statistical model is still a collection of distributions, but now the assumptions on the queries, actions, and data samples can be relaxed in various ways.  For example, rather than assuming each data point is iid, perhaps it is iid condition on the previous $k$ samples, yielding a Markov model. More generally, one could assume that each is governed by a  stochastic processes. A stochastic process, $\{X(t) : t \in T \}$, where $T = [0,\infty)$, can be thought of as a collection of random variables each indexed by time $t$. So, for example, rather than assuming each sample $s_t$ is an observation of some fixed random variable $S$, each sample $s_t$ is an observation from the stochastic process $\{S(t): t \in T \}$.
    % 
    % \item 
    \paragraph{Feedback} $\mc{V}$.  In batch learning, each query/action pair had an associated risk.  In sequential learning,  we potentially get feedback $V_i \in \mc{V}$ associated with any action we take.  In general, this feedback could be what the best action to take was, $Y_i^*$, or the loss incurred by taking $\hat{Y}_i$, or something else.  This feedback may be errorful, and is a function of the query, action, true distribution, and risk.  
        % 
    % \item 
    \paragraph{Learners}, $\mc{F} \subseteq \{f: \cH' \times \mc{S}^* \times \mc{V} \times \Lambda \mapsto \cH'\}$. This definition differs from the previous definition by including two additional inputs: a hypothesis,  $h \in \cH' \subseteq \cY^\cX$ (interpreted as a previous hypothesis), and feedback $v \in \mc{V}$. The output of $f$ is another hypothesis that can be thought of as an updated version of the input hypothesis. 
    % 

    % \item 
    \paragraph{Error} $\cE$. In sequential learning scenarios, we are often  interested in the sum of expected excess risks, or \textbf{cumulative expected regret}:
\begin{align} \label{XAeq:cer}
    % \mc{E}_f(\D) = 
    \sum_n \left( \mbb{E}[R(\hat{h}_n)] - R' \right),
\end{align}
where $R'$ is the risk of the best fixed hypothesis in hindsight. 
% \end{itemize}
% 

\begin{definition}[Round]
    %  
Given the above changes, we can introduce the concept of a \textbf{round}. A round is typically defined by the following sequence of events for the learner: 
    \begin{enumerate}
        \item receive a query $X_i$,
        \item receive a data sample $S_i$ (potentially chosen adversarially), 
        \item choose a hypothesis $\hat{h}_i \in \cH$,
        \item take action $\hat{h}(X_i) = \hat{Y}_i$,
        \item receive feedback $V_i$, and
        \item update hypothesis, $\hat{h}_{i+1} \leftarrow f(\hat{h}_i, S_i, V_i)$.  
    \end{enumerate}

\end{definition}


Note that in the above, unlike in the batch learning setting, we often do not assume that each data point $S_i$ is sampled identically and independently from the same fixed but unknown distribution $P_S \in \cP_S$. Rather, in sequential learning, each data point can be sampled from a potentially dynamic, non-stationary, or even adversarial distribution, $P^S_i$. Moreover, although a round typically is assumed to consist of each of the above steps, in general, a round may not include any of them.  For example, feedback might be deferred until many steps have been taken, or the learner $f$ may receive several queries without taking any actions. 

\subsection{Sequential Learning Tasks}

Here we provide three canonical sequential learning paradigms. 

\begin{example}[Online Learning]
    Any of the above learning scenarios can be either batch or online, including point estimation, hypothesis testing, supervised learning, and unsupervised learning. The main differences when we move from batch to online learning is using stochastic processes rather than random variables to define the model assumptions, and that the error is typically cumulative expected regret, rather than expected risk or expected excess risk. In other words, we can think of online learning as generalizing batch learning in that instead of each sample being from the same distribution, each sample can come from a different distribution. %Typically in online learning, each round consists of each of the six steps enumerated above. 
\end{example}

\begin{example}[Reinforcement Learning]
    Reinforcement learning can be thought of as a generalization of online learning described above. Specifically, in reinforcement learning, each step of a given round is optional, that is, the learner $f$ might not receive data, a query, take an action, or receive feedback at any given round. For example, when playing a game, the learner $f$ may only receive feedback at the very end of a game after many rounds. 
\end{example}


\begin{example}[Streaming Learning]
Streaming learning is related to online learning, with a twist.  In streaming learning, there are also rounds, as the data either arrive sequentially or may simply be operated on sequentially for computational reasons.  However, the model is not a collection of stochastic processes, rather, merely a collection of random variables.  Thus, for instance, the distribution of data is iid, so $P_i = P\,  \forall i$. This also means that the optimal hypothesis is the same for each round, $h^*_i = h^* \, \forall i$.  But streaming learning has an additional property: the computation complexity is  \textit{bounded} in streaming learning. 
If it were not constrained, then $f$ (or $h$) could store all the data it has seen, and retrain with each new sample.  Such a strategy would na\"ively require $\mc{O}(n)$ space and $\mc{O}(n^2)$ time.  Therefore, for $f$ to be a streaming learner, it must be computationally bounded.  The least restrictive space and time constraints would be $f=o(n)$ space and/or $f=o(n^2)$ time.  More commonly, $f=\mc{O}(1)$ space and time (recall, we assume that $h$ is constrained in the same way as $f$, otherwise it could do all the work). Note that batch, online, and reinforcement learning can each incorporate computational complexity bounds, in which case each would become a streaming learning scenario. 
\end{example}



% \begin{example}[Vertex Nomination]
%     The query space $\mc{X} = V \times 2^{V \backslash \{v^*\}}$, where $2^A$ is the power set of $A$. A query is a vertex of interest (VOI) $v^* \in V$ with an associated subset of similar vertices $S \in 2^{V \backslash \{v^*\}}$. The action space $\mc{Y} = 2^{V \backslash \{v^*\}}$, which is also the set of all possible values for $S'$, the full set of similar nodes. $\mc{H}$ can contain any $h: \mc{X} \mapsto \mc{Y}$, but can be restricted to those that say embed the nodes $V$ into Euclidean space and return the nodes that are close in this space. There are multiple choices of the risk $R$, such as
%     \begin{align*}
%         R(h) = \E{}{\Delta(h(v^*, S), S')},
%     \end{align*}
%     where $\Delta(\cdot, \cdot)$ is some set distance such as intersection-over-union (IoU). Each data point is an edge, making the data space $\{\{u, v\} : u, v \in V \text{ and } u \neq v\}$, or the set of all possible edges. Finally, an example of $\cF$ all learning algorithms that produce an embedding of $V$ such that the distance between $v^*$ and any $v \in S$ is small, and use that embedding in any learned hypothesis.
% \end{example}


\subsection{A hierarchy of task}
\label{app:hier}

The `simplest' form of learning is \textit{batch learning}, which includes as special cases: point estimation, hypothesis testing, supervised learning, unsupervised learning, and causal learning.  In batch learning the learner faces a single setting and distribution.  \textit{Sequential learning} generalizes batch learning by enabling many sequential rounds of learning, which requires that the learner continually updates its hypothesis to effectively learn. Special cases of sequential learning in streaming learning, online learning, and reinforcement learning.  All of the aforementioned learning scenarios are \textit{in-distribution task learning} scenarios, and have a single setting, with a single fixed goal.  In general, any of them may also have computational complexity constraints, in which case the task learners typically learn compressed internal representations with which to operate on.  In online learning and reinforcement learning it is often ambiguous whether there is only a single task or not. Here, we propose a solution to this conundrum: to count as a new task, something in the setting must change, rather than merely the distribution of samples, queries, or actions.  

Note that often people assert that there are three different kinds of in-distribution single task learning scenarios: unsupervised learning, supervised learning, and reinforcement learning.  One can obtain such a classification from our definitions as follows.  First, treat point estimation as unsupervised learning. This follows because point estimation is a special kind of unsupervised learning where the actions are parameters of a distribution, rather than say, cluster assignments or low-dimensional manifolds.  Second, treat hypothesis testing as supervised learning.  Again, this makes sense upon further inspection. Consider two-sample testing for example (which can be used to solve quite general hypothesis testing scenarios~\cite{Panda2020-vc}).  Which `sample' a given data point is associated with can be considered the label.  Third, treat causal learning as a special case of supervised learning, which requires additional assumptions.  Finally, treat all versions of sequential learning as  special cases of reinforcement learning.  Thus,  our taxonomy is not inconsistent with the (unsupervised, supervised, reinforcement) learning taxonomy, rather, it can be thought of as a refinement of it.  


All the remaining kinds of learning we have discussed are all special cases of {out-of-distribution learning}.  \textit{Transfer learning} is the simplest generalization of batch learning: there is still only one task, but now there are multiple datasets.  As we previously mentioned, prior knowledge, previously learned hypotheses, and even inductive biases of the learner and/or hypotheses can reasonably be considered datasets in their own right, indicating that even in-distribution learning can be accurately viewed as transfer learning as well.  \textit{Multitask learning} generalizes transfer learning by introducing additional tasks; the learners job becomes transferring omni-directionally between all tasks~\cite{pl}. Meta-learning further introduces additional as yet unobserved tasks, so the learner must `learn-to-learn' in order to improve performance on these tasks, over and above what its performance would have been without learning on the observed tasks. Continual learning introduces a sequential distribution over tasks.  Moreover, continual learning also requires computational complexity constraints, lest a learner could simply perform multitask or meta-learning after each new data sample arrives.  Finally, lifelong learning adds dynamic priorities and constraints, to reflect the realities of actual agents developing, being adults, and then aging. Each of the out-of-distribution learning tasks can each consist of multiple tasks of any kind, including batch and/or sequential learning.  

\subsubsection{Self-supervised, zero-shot, few-shot, and domain adaptation}


There are a number of popular learning paradigms currently in the literature that we have basically not  discussed, including self-supervised, zero-shot, few-shot, and out-of-distribution learning.  Nonetheless, our framework is sufficient to incorporate those as well.  Self-supervised is a kind of multitask learning, where each task is constructed to be unsupervised learning, typically applied to structured data (such as sequences)~\cite{Doersch2017-ez}. Zero-shot~\cite{Socher2013-eo} (also called zero-resource~\cite{Renshaw2015-ue}) and few-shot~\cite{Snell2017-jj} learning can be any kind of out-of-distribution learning, though is typically discussed in a transfer learning setting.  The key difference between zero-shot and few-shot learning, and other forms of transfer learning, is in zero- and few-shot learning we are particularly interested in learning efficiency when the new dataset, $\D^{M+1}$, has small cardinality, potentially even zero samples. Because classical definitions of learning have minimal sample sizes to determine whether or not a learner has learned, they are not appropriate in such contexts.  
Domain adaptation is another form of transfer learning~\cite{Daume2007-cv} in which the learner explicitly attempts to adjust for the difference between the source and target distributions.  


==> extra/machine_learning.tex <==



\section{Definitions of In-Distribution Learning} 
\label{app:def}
% 
\citet{Shalev-Shwartz2014-zo} discuss three alternative definitions of learning. We restate them here with slight notational modifications.  For each definition, we will leverage a notion of convergence for random variables, which is required because  the risk of the learner is a random variable~\cite{Bickel1993-wz}. A sequence $\{X_n\}$ of random variables converges in probability towards the random variable $X$ if for all $\eps,\delta > 0$, there exists an $N(\eps,\delta) \in \mbb{N}$ such that 
$$\mbb{P}[|X_n - X| \leq \eps ] \geq 1 - \delta, \quad \forall n \geq N(\eps,\delta) \enspace .$$

Each of the below definitions are in-distribution definitions of learning, so they have implicitly assumed when they write $P$, that the distribution of queries is about the distribution that the data are assumed to be sampled from. 


% 
\begin{definition}[Agnostic PAC Learnability]
A hypothesis class $\cH$ is agnostically PAC learnable if there exists a learning algorithm $f$, and a function $N : (0,1)^2 \mapsto \mathbb{N}$ such that, 
for all $\eps, \delta >0 $ and for every distribution $P$, if  each $S_i \iid P$, then it holds that 
% 
$$\mbb{P}[R(\hat{h}_n) - R^\diamond \leq \eps] \geq 1 - \delta, \quad \forall n \geq N(\eps,\delta),$$
which implies that
$$  \mbb{P}[R(\hat{h}_n) -  R(h) \leq \eps] \geq 1 - \delta, \quad \forall h \in \cH, \, \forall \eps,\delta > 0 , \forall P, \forall n \geq N(\eps,\delta).$$
If $f$ runs in time polynomial in $\eps$, $\delta$, $n$, $d$, and $size(h)$,  where $d$ is the dimensionality of $x$, that is, $\mc{X} \subseteq \Real^d$, and  $size(h)$ is the maximal cost of the computational representation of $h \in \cH$, then we say $f$ efficiently learns for the given problem. 
\end{definition}



The above definition both defines PAC learnable problems (those for which a learner $f$ exists that satisfies the above conditions), and also defines whether a particular $f$ learns in a particular problem (if $f$ achieves those bounds for that problem, then it learns that problem). Implicit in the above definition is that the distribution of samples (training data) is the same as the distribution the learned hypothesis will be evaluated on (i.e., the distribution of the query/action pairs). Not all problems are PAC learnable, however, some are 'harder'. Nonuniform learnability is a generalization of PAC learnability.
% 
\begin{definition}[Nonuniform Learnability]
A hypothesis class $\cH$ is nonuniformly learnable if 
there exists a learning algorithm $f$,
and a function $N : (0,1)^2 \times \cH \mapsto \mathbb{N}$,
such that if $S_i \iid P$, then it holds that 
$$ \mbb{P}[R(\hat{h}_n) -  R(h) \leq \eps] \geq 1 - \delta, \quad  \forall h \in \cH, \, \forall \eps, \delta > 0, \, \forall \, P, \, \forall n \geq N(\eps,\delta,h).$$
\end{definition}

The main difference between PAC learning and Nonuniform learning is in nonuniform learning, the minimum sample size $N$ can depend on the particular hypothesis $h$ of interest, whereas for PAC learning, the sample size is the same for all $h$.

There are a few points to highlight about both of these definitions of learning.  First, whether or not $f$ learns is a function not just of a specific $h$, but of all $h \in \cH$.  Second, one can only ascertain whether $f$ has learned if the sample size is large enough. Third, there are no distributional assumptions (other than iid).   

Consistency is a complementary notion of learning. Informally, we say that a learner is \textit{consistent} with respect to a distribution $P$ if it asymptotically achieves the minimum. 

% 
\begin{definition}[Consistency]
A learner $f$ is consistent for statistical model $\cP$ if there exists a function $N:(0,1)^2 \times \mc{P} \mapsto \mbb{N}$, where it holds that 
$$\mbb{P}[R(\hat{h}_n)  - R^* \leq \eps ] \geq 1 - \delta, \quad \eps,\delta>0, \, \forall P \in \cP, \,  \forall n > N(\eps,\delta,P).$$

A learner is \textbf{universally consistent} if it achieves the minimum for any statistical model $\cP$, that is, for any possible distribution $P$: 
$$\mbb{P}[R(\hat{h}_n)  - R^* \leq \eps ] \geq 1 - \delta, \quad \eps,\delta \in (0,1) , \, \forall P, \,  \forall n > N(\eps,\delta,P).$$
\end{definition}


Consistency differs from PAC and non-uniform learnability in a key way.  Consistency does not restrict the decision rule to be from a specific class $\cH$, whereas PAC and non-uniform learnability do\footnote{Note that~\citet{Shalev-Shwartz2014-zo} does include $\cH$ in their definition of consistency, but that is not a common practice.}. Instead, consistency is limited only to a subset of distributional assumptions (such as Gaussian).  All three definitions, however, share a few key properties.  First, to assert that  an $f$ learns in some scenario requires sample size being sufficiently large.  This renders them impractical for theoretically characterizing zero-shot or few-shot learning, including many real biological learning scenarios.  Second, to claim an $f$ learns requires comparing to some notion of optimality.  Biologically, agents often learn to adequacy, rather than optimality.  Third, there is only a single dataset, distribution, and task.  In multi-task learning, meta-learning,  and biological learning, there are  multiple datasets, distributions, and tasks. Thus, although the framework described in this section is quite powerful and general, it is inadequate to characterize learning in various modern and biological out-of-distribution learning scenarios.  See Appendix~\ref{app:classic} for a formal treatment of several in-distribution learning problems using this notation. 



==> extra/task_awareness.tex <==


The following instantiates task awareness, obliviousness, and agnosticism in the context of binary classification. Let $\mc{X} = \R^d$, $\mc{Y} = \{-1, 1\}$, and let $\mc{T}$ = the spaces of tasks. For each task $t \in \mc{T}$, the decision problem is to map a random point $X$ to its class label $Y$, when $(X, Y) \sim P_{XY}^{(t)}$, some distribution governed by the task $t$. While more generally the tasks can differ in any way (see Section \ref{sec:framework}), for us, they will only differ in the distribution $P_{XY}^{(t)}$ on $\mc{X} \times \mc{Y}$ that the input-label pairs follow given $t$.

There are six types of task specification - the product space of the three forms of labelling as well as whether the tasks are revealed at test time versus train time.

\subsection{Task Aware Decision Problem}

A test point $(X, Y) \sim P_{X, Y}^{(t)}$ is drawn from a distribution associated to task $t \in \mc{T}$. A hypothesis $h: \mc{X} \times \mc{T} \rightarrow \mc{Y}$ in hypothesis class $\mc{H}$ consumes a test point $X$ and associated task label $t$ and classifies it as $\hat{Y} = h(X, t)$.

\subsection{Task Aware Learning}

Training examples $(X_i, Y_i, t_i) \sim P_{X, Y}^{(t_i)}$ are drawn independently but not identically distributed for $i = 1, ..., n$, each from a distribution dependent on the task $t_i$ associated to that example. A learning algorithm $f: (\mc{X} \times \mc{Y} \times \mc{T})^n \rightarrow \mc{H}$ consumes $n$ input-label-task triples and outputs a learned hypothesis $\hat{h} = f(\{X_i, Y_i\}_{i=1}^n)$.

\subsection{Task Oblivious Decision Problem}

A test point $(X, Y) \sim P_{X, Y}^{(t)}$ is drawn from a distribution associated to task $t \in \mc{T}$. A hypothesis $h: \mc{X} \rightarrow \mc{Y}$ in hypothesis class $\mc{H}$ consumes a test point $X$ with no task label and classifies it as $\hat{Y} = h(X)$.

\subsection{Task Oblivious Learning}

Training examples $(X_i, Y_i, t_i) \sim P_{X, Y}^{(t_i)}$ are drawn independently but not identically distributed for $i = 1, ..., n$, each from a distribution dependent on the task $t_i$ associated to that example. A learning algorithm $f: (\mc{X} \times \mc{Y})^n \rightarrow \mc{H}$ consumes $n$ input-label pairs (with no task) and outputs a learned hypothesis $\hat{h} = f(\{X_i, Y_i\}_{i=1}^n)$.

\subsection{Task Agnostic Decision Problem}

Let $\mc{T}' = \mc{T} \cup \{\text{null}\}$, where ``null" indicates an unknown task. A test point $(X, Y) \sim P_{X, Y}^{(t)}$ is drawn from a distribution associated to task $t \in \mc{T}$. A hypothesis $h: \mc{X} \times \mc{T}' \rightarrow \mc{Y}$ in hypothesis class $\mc{H}$ consumes a test point $X$ and associated task label $t' \in \mc{T}'$ (that can be null) and classifies it as $\hat{Y} = h(X, t')$.

\subsection{Task Agnostic Learning}

As before, let $\mc{T}' = \mc{T} \cup \{\text{null}\}$, where ``null" indicates an unknown task. Training examples $(X_i, Y_i, t_i) \sim P_{X, Y}^{(t_i)}$ are drawn independently but not identically distributed for $i = 1, ..., n$, each from a distribution dependent on the task $t_i$ associated to that example. A learning algorithm $f: (\mc{X} \times \mc{Y} \times \mc{T}')^n \rightarrow \mc{H}$ consumes $n$ input-label-task pairs (with the task field potentially being ``null") and outputs a learned hypothesis $\hat{h} = f(\{X_i, Y_i, t'_i\}_{i=1}^n)$.

==> ll_input.tex <==
\clearpage 


% \begin{align}
% % \text{trained model :=} 
% \hat{h}_n  = \underbrace{g}_{\text{learner}} \big( \underbrace{(X,Y)_n }_{\text{training data}} \big).
% \end{align}



% \begin{align}
% % \text{loss function:=} 
% \ell(f(X),Y). 
% \end{align}


\begin{align}
% \text{risk :=} 
R(f) =  \underbrace{\int_{(\cX,\cY)}}_{\text{possible test}} 
\underbrace{\ell(f(X),Y)}_{\text{loss function}}
\underbrace{dP_{X,Y}}_{\text{distribution}}.
\end{align}


% \begin{equation}
%     \begin{split}
%     \end{split}
% \end{equation}
\begin{align}
% classical 
\mathcal{E}_{\text{classical}} \left(f, n, P \right)
=&
     \underbrace{\int_{(\cX,\cY)_n}}_\text{possible train}  
     \underbrace{R(f)}_{\text{risk}} 
     \underbrace{dP_{(X,Y)_n}}_\text{distribution}
% \\
=&  \underbrace{\int_{(\cX,\cY)_n}}_\text{possible train}  
    \underbrace{\int_{(\cX,\cY)}}_{\text{possible test}} 
\underbrace{\ell(f(X),Y)}_{\text{loss function}}
\underbrace{dP_{X,Y}}_{\text{distribution}}     \underbrace{dP_{(X,Y)_n}}_\text{distribution}.
\end{align}

\begin{align}
% OOD 
\mathcal{E}_{\text{OOD}} \left(f,n, {\color{red}{P^{\text{test}}, P^{\text{train}}}} \right)
=&  \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{train}}}}}_\text{possible train}  
    \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{test}}}}}_{\text{possible test}} 
\underbrace{\ell_{\color{red}{\text{test}}}(f(X),Y)}_{\text{loss function}}
\underbrace{d \color{red}{P^{\text{test}}_{X,Y}}}_{\text{distribution}}     
\underbrace{d \color{red}{P^{\text{train}}_{X,Y}}}_{\text{distribution}}.
\end{align}


\begin{align}
% continual 
\mathcal{E}_{\text{continual}} \left( h, n, {\color{red}{P^{\text{future, past}}}} \right)
=&  \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{past}}}}}_\text{possible past}  
    \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{future}}}}}_{\text{possible future}} 
\underbrace{\ell_{\color{red}{\text{future}}}(f(X),Y)}_{\text{loss function}}
\underbrace{d \color{red}{P^{\text{future | past}}_{X,Y}}}_{\text{distribution}}     
\underbrace{d \color{red}{P^{\text{past}}_{X,Y}}}_{\text{distribution}}
\end{align}


\begin{align}
% causal 
\mathcal{E}_{\text{causal}} \left( {\color{red}{\text{do}(f)}}, n, P \right)
=&  \underbrace{\int_{(\cX,\cY)_n}}_\text{possible train}  
    \underbrace{\int_{(\cX,\cY)}}_{\text{possible test}} 
\underbrace{\ell({\color{red}{\text{do}}}(f(X)),Y)}_{\text{loss function}}
\underbrace{dP_{X,Y}}_{\text{distribution}}     \underbrace{dP_{(X,Y)_n}}_\text{distribution}
% \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{past}}}}}_\text{possible past}  
%     \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{future}}}}}_{\text{possible future}} 
% \underbrace{\ell_{\color{black}{\text{future}}}(f(X), {\color{red}{\text{do}(Y)}})}_{\text{loss function}}
% \underbrace{d \color{red}{P^{\text{future | past}}_{X,Y}}}_{\text{distribution}}     
% \underbrace{d \color{red}{P^{\text{past}}_{X,Y}}}_{\text{distribution}}
\end{align}



\begin{equation*}
\begin{split}
% causal 
\text{minimize } 
&\mathcal{E}_\text{prospective} \left(\text{do}(f), n, P^{\text{future, past}} \right),  
\\
\text{subject to } &f \in \mathcal{F}_\text{prospective}
\\ \text{and } & P^\text{future, past} \in \mathcal{P}_{\text{prospective}}
\end{split}    
\end{equation*}


where

\begin{align*}
% prospective 
\mathcal{E}_{\text{prospective}} \left( {\color{black}{\text{do}(f)}}, n, {\textcolor{black}{P^{\text{future, past}}}}  \right)
=&  \underbrace{\int_{(\cX,\cY)_{\color{black}{\text{past}}}}}_\text{possible past}  
    \underbrace{\int_{(\cX,\cY)_{\color{black}{\text{future}}}}}_{\text{possible future}} 
\underbrace{\ell_{\color{black}{\text{future}}}( {\color{black}{\text{do}(f(X))}}, Y)}_{\text{loss function}}
\underbrace{d \color{black}{P^{\text{future | past}}_{X,Y}}}_{\text{distribution}}     
\underbrace{d \color{black}{P^{\text{past}}_{X,Y}}}_{\text{distribution}}
\end{align*}

\begin{align*}
% prospective 
\mathcal{E}_{\text{prospective}} \left( {\color{red}{\text{do}(f)}}, n, {\textcolor{red}{P^{\text{future, past}}}}  \right)
=&  \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{past}}}}}_\text{possible past}  
    \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{future}}}}}_{\text{possible future}} 
\underbrace{\ell_{\color{black}{\text{future}}}( {\color{red}{\text{do}(f(X))}}, Y)}_{\text{loss function}}
\underbrace{d \color{red}{P^{\text{future | past}}_{X,Y}}}_{\text{distribution}}     
\underbrace{d \color{red}{P^{\text{past}}_{X,Y}}}_{\text{distribution}}
\end{align*}






% \begin{align}
%     P_{X,Y}^\text{past} = P_{X_0} \prod_{t=1}^n P_{X_t | X_{t-1}}
% \end{align}

% \begin{align}
%     P_{X,Y}^\text{past} = P_{X_0} \prod_{t=1}^n P_{X_t | X_{t-1}, Y_{t-1}}
% \end{align}


% \begin{align}
% \mathcal{E}_{\text{prospective}} \left(g; X,{\color{red}{\text{do}(Y)}} \right) =&  \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{past}}}}}_\text{possible past}  
%     \underbrace{\int_{(\cX,\cY)_{\color{red}{\text{future}}}}}_{\text{possible future}} 
% \underbrace{\ell_{\color{black}{\text{future}}}(f(X), {\color{red}{\text{do}(Y)}})}_{\text{loss function}}
% \underbrace{d \color{red}{P^{\text{future | past}}_{X,Y}}}_{\text{distribution}}     
% \underbrace{d \color{red}{P^{\text{past}}_{X,Y}}}_{\text{distribution}}
% \end{align}


% $\argmin_{g \in \mc{G}} \mathcal{E}_{\text{causal}}$

% \begin{align}
%     \text{LE}_f( {\color{red}{D_{care}}},{\color{green}{D_{other}}})= \frac{ {\color{yellow}{\mathcal{E}_f}}({\color{red}{D_{care}}}) }{ {\color{yellow}{\mathcal{E}_f}}({\color{red}{D_{care}}} \cup {\color{green}{D_{other}}})}
% \end{align}

==> macros_jmlr.tex <==
\usepackage{mathtools}
\providecommand{\RR}{\Gamma} %real numbers
\newcommand{\Nat}{I\!\!N} %natural numbers

\newcommand{\cT}{\mathcal{T}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cK}{\mathcal{K}}

\newcommand{\T}{\mathbf{T}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\renewcommand{\P}[2]{P_{#1}\left[#2\right]}
\newcommand{\I}[2]{\mathbb{I}_{#1}\left\{#2\right\}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\indep}{\raisebox{0.05em}{\rotatebox[origin=c]{90}{$\models \;$}}}
\newcommand{\up}[1]{^{(#1)}}

\newcommand{\TE}{\text{TE}}
\newcommand{\ME}{\text{ME}}
\newcommand{\LE}{\mathsf{LE}}
\newcommand{\LLE}{\text{LLE}}
\newcommand{\FTE}{\text{FTE}}
\newcommand{\BTE}{\text{BTE}}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}


\newtheorem{application}{Application}[section]

\newcommand{\D}{\mathbf{D}}


\newcommand{\comE}[1]{{\color{red}ERIC: #1}}

==> nd_preamble_jmlr.tex <==
%===============================================================================%
% This is the neurodata latex preamble.
%
% We have desigend it to augment the SIAM LaTeX2e Multimedia Macros for
% Online-Only Journals, located here:
% https://www.siam.org/Portals/0/Macros/Online/siamonline_190516.zip
%
% If you need a specific package please load it here.
%===============================================================================%

% \usepackage{comment}
% \usepackage{lipsum}
% \usepackage[margin=1in, footskip=36pt]{geometry}
% 
% %%% For author, thanks, affil
% %\usepackage[noblocks]{authblk}
% \usepackage{endnotes}
% \renewcommand{\notesname}{Affiliations}
% 
% \usepackage{titlesec}
% \usepackage{titletoc}
% \usepackage{pgfplotstable}
% %%=================
% %% Define Headings and section task
% %%=================
% \titleclass{\task}{straight}[\section]
% \newcounter{task}
% \renewcommand{\thetask}{\arabic{task}}
% \titleformat{\task}[hang]
%     {\normalfont\LARGE\bfseries}{Task \thetask:}{1em}{}
% 
% 
% \titleformat*{\task}{\color{header1}\bfseries}
% 
% \titlecontents{task}
%               [3.8em] % ie, 1.5em (chapter) + 2.3em
%               {}
%               {\contentslabel{2.3em}}
%               {\hspace*{-2.3em}}
%               {\titlerule*[1pc]{.}\contentspage}
% 
% 
% \titlespacing*{\section}{0ex}{1ex}{1ex}
% \titlespacing*{\subsection}{0ex}{1ex}{1ex}
% \titlespacing*{\subsubsection}{0ex}{1ex}{1ex}
% \titlespacing*{\paragraph}{0ex}{1ex}{1ex}
% \titlespacing*{\subparagraph}{0pt}{1ex}{1ex}
% \titlespacing*{\task}{0em}{1ex}{1ex}
% 
% 
% %%% for footnote affiliation block
% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }
% 
% %%% Bib and citations
% \usepackage[sort&compress,comma,square,numbers]{natbib}
% 
% %%% mathfonts, equation environments and eqref, ...
% \usepackage{amsfonts,amsmath,amssymb}
% \usepackage{bbm}
% 
% %%% For enumitem with special global options
% \usepackage{multicol}
% \usepackage{enumitem}
% \setlist[enumerate]{wide, labelindent=1cm,  noitemsep}
% % \setlist[enumerate]{noitemsep}
% \setlist[itemize]{noitemsep}
% \setlist[description]{noitemsep}
% 
% %%% For colors and sout and hhlines
% \usepackage{hhline}
% 
% %%%%%%%%%%% EDITING MACROS %%%%%%%%%%%%%
% \usepackage{todonotes}
% \RequirePackage{ulem}
% \newcommand{\add}[1]{\textcolor{blue}{[#1]}}
% \newcommand{\rep}[2]{\textcolor{brown}{[\sout{#1} $|$ #2]}}
% \newcommand{\dele}[1]{\textcolor{red}{\sout{#1}}}
% 
% %% Set up Tables
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%===%
% \definecolor{tableheadcolor}{gray}{0.92}
% % Following is taken from Werner: http://tex.stackexchange.com/a/33761/3061
% % and modified for my needs
% %
% % Command \topline consists of a (slightly modified)
% % \toprule followed by a \heavyrule rule of colour tableheadcolor
% % (hence, 2 separate rules)
% \newcommand{\topline}{ %
%         \arrayrulecolor{blue1}\specialrule{0.1em}{\abovetopsep}{0pt}%
%         \arrayrulecolor{tableheadcolor}\specialrule{\belowrulesep}{0pt}{0pt}%
%         \arrayrulecolor{blue1}}
% % Command \midline consists of 3 rules (top colour tableheadcolor, middle colour black, bottom colour white)
% \newcommand{\midtopline}{ %
%         \arrayrulecolor{tableheadcolor}\specialrule{\aboverulesep}{0pt}{0pt}%
%         \arrayrulecolor{blue1}\specialrule{\lightrulewidth}{0pt}{0pt}%
%         \arrayrulecolor{white}\specialrule{\belowrulesep}{0pt}{0pt}%
%         \arrayrulecolor{blue1}}
% % Command \bottomline consists of 2 rules (top colour
% \newcommand{\bottomline}{ %
%         \arrayrulecolor{white}\specialrule{\aboverulesep}{0pt}{0pt}%
%         \arrayrulecolor{blue1} %
%         \specialrule{\heavyrulewidth}{0pt}{\belowbottomsep}}%
% 
% 
% \newcommand{\midheader}[2]{%
%         \midrule\topmidheader{#1}{#2}}
% \newcommand\topmidheader[2]{\multicolumn{#1}{c}{\textsc{#2}}\\%
%                 \addlinespace[0.5ex]}
% 
% \pgfplotstableset{normal/.style ={%
%         header=true,
%         string type,
%         font=\small,
%     	column type={p{.092\textwidth}},
%         every head row/.style={
%             before row={\topline\rowcolor{tableheadcolor}},
%             after row={\midtopline}
%         },
%         every odd row/.style={
%             before row={\rowcolor{blue1}}
%         },
%         every last row/.style={
%             after row=\bottomline
%         },
%         col sep=&,
%         row sep=\midrule
%     }
% }
% 
% \usepackage{multirow}
% 
% 
% %%% for \toprule
% \usepackage{booktabs}
% \usepackage{titlesec}
% \usepackage{fancyhdr}
% \usepackage{fullpage}
% 
% % Define LaTeX friendly Fonts
% %==============
% \RequirePackage{titlesec}
% \RequirePackage[font={footnotesize},{singlelinecheck=false}]{caption}
% \captionsetup{belowskip=-5pt}
% 
% \usepackage[T1]{fontenc}
% \usepackage[scaled]{helvet}
% \usepackage[scaled=1.10, med]{zlmtt}
% \renewcommand\familydefault{\sfdefault}
% 
% 
% %%% For begin{algorithm}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% 
% \newcommand{\Linefor}[2]{%
%     \State \algorithmicfor\ {#1}\ \algorithmicdo\ {#2} \algorithmicend\ \algorithmicfor%
% }
% \newcommand{\Lineif}[2]{%
%     \State \algorithmicif\ {#1}\ \algorithmicdo\ {#2} \algorithmicend\ \algorithmicif%
% }
% 
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%% MACROS %%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% 
% %%%%%%%%%%% ALGORITHM NAMES %%%%%%%%%%%%%
% \providecommand{\sct}[1]{{\sc \texttt{#1}}}
% 
% \newcommand{\Idt}{\sct{Idt}}
% \newcommand{\Svd}{\sct{Svd}}
% \newcommand{\Pca}{\sct{Pca}}
% \newcommand{\Fld}{\sct{Fld}}
% \newcommand{\Lda}{\sct{Lda}}
% \newcommand{\eig}{\sct{eig}}
% \newcommand{\Lol}{\sct{Lol}}
% \newcommand{\Lal}{\sct{Lal}}
% \newcommand{\Qoq}{\sct{Qoq}}
% \newcommand{\Lrl}{\sct{Lrl}}
% \newcommand{\Lfl}{\sct{Lfl}}
% \newcommand{\Faq}{\sct{Faq}}
% \newcommand{\qr}{\sct{qr}}
% 
% \newcommand{\Mgc}{\sct{Mgc}}
% \newcommand{\Mgcp}{\Mgc$_P$}
% \newcommand{\Mgcd}{\Mgc$_D$}
% \newcommand{\Mgcm}{\Mgc$_M$}
% \newcommand{\Hhg}{\sct{Hhg}}
% \newcommand{\Dcorr}{\sct{Dcorr}}
% \newcommand{\Dcov}{\sct{Dcov}}
% \newcommand{\Mcorr}{\sct{Mcorr}}
% \newcommand{\Mantel}{\sct{Mantel}}
% \newcommand{\Mic}{\sct{Mic}}
% \newcommand{\Hsic}{\sct{Hsic}}
% \newcommand{\Pearson}{\sct{Pearson}}
% \newcommand{\Kendall}{\sct{Kendall}}
% \newcommand{\Spearman}{\sct{Spearman}}
% \newcommand{\RV}{\sct{RV}}
% \newcommand{\CCA}{\sct{Cca}}
% \newcommand{\Sporf}{\sct{Sporf}}
% \newcommand{\Mf}{\sct{Mf}}
% \newcommand{\MF}{\sct{RF}}
% \newcommand{\ICC}{\sct{ICC}}
% 
% 
% 
% %%%%%%% MATH OPERATORS %%%%%%%%%%%%
% 
% \providecommand{\ve}[1]{\boldsymbol{#1}}
% \providecommand{\ma}[1]{\boldsymbol{#1}}
% \providecommand{\deter}[1]{\lvert #1 \rvert}
% \newcommand{\argmax}{\operatornamewithlimits{argmax}}
% \newcommand{\argmin}{\operatornamewithlimits{argmin}}
% \newcommand{\argsup}{\operatornamewithlimits{argsup}}
% \newcommand{\arginf}{\operatornamewithlimits{arginf}}
% \newcommand{\T}{^{\ensuremath{\mathsf{T}}}} % transpose
% \providecommand{\norm}[1]{\ensuremath{\left \lVert#1 \right  \rVert}}
% \providecommand{\abs}[1]{\ensuremath{\left \lvert #1 \right \rvert}}
% % \providecommand{\mat}[1]{\left[ #1 \right]}
% % \newcommand{\trans}[1]{{#1}^{\ensuremath{\mathsf{T}}}}    % \newcommand{\transpose}[1]{{#1}^{\ensuremath{\mathsf{T}}}}
% \newcommand{\from}{{\ensuremath{\colon}}}           % :
% \newcommand{\trace}[1]{{\ensuremath{\operatorname{tr}\!\left(#1\right)}}}           % :
% %

\usepackage{xcolor}

\providecommand{\mc}[1]{\mathcal{#1}}
% \providecommand{\tmc}[1]{\tilde{\mathcal{#1}}}
\providecommand{\mb}[1]{\boldsymbol{#1}}
\providecommand{\ms}[1]{\mathsf{#1}}
\providecommand{\mt}[1]{\widetilde{#1}}
\providecommand{\mbb}[1]{\mathbb{#1}}
\providecommand{\mv}[1]{\vec{#1}}
\providecommand{\mh}[1]{\hat{#1}}
\providecommand{\wh}[1]{\widehat{#1}}
\providecommand{\mhv}[1]{\mh{\mv{#1}}}
\providecommand{\mvh}[1]{\mv{\mh{#1}}}
\providecommand{\mhc}[1]{\hat{\mathcal{#1}}}
% \providecommand{\mbc}[1]{\mb{\mathcal{#1}}}
% \providecommand{\mvc}[1]{\mv{\mathcal{#1}}}
% \providecommand{\mtc}[1]{\widetilde{\mathcal{#1}}}
% \providecommand{\mth}[1]{\mt{\mh{#1}}}
% \providecommand{\mht}[1]{\mh{\mt{#1}}}
% \providecommand{\mhb}[1]{\hat{\boldsymbol{#1}}}
% \providecommand{\whb}[1]{\widehat{\boldsymbol{#1}}}
% \providecommand{\mvb}[1]{\vec{\boldsymbol{#1}}}
% \providecommand{\mtb}[1]{\widetilde{\boldsymbol{#1}}}
% \providecommand{\mbt}[1]{\widetilde{\boldsymbol{#1}}}
% \providecommand{\mvc}[1]{\vec{\mathcal{#1}}}
% % \newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
% \newcommand{\dd}[2]{\frac{\partial ^2 #1}{\partial #2 ^2}}
% \newcommand{\DDD}[3]{\frac{\partial ^2 #1}{\partial #2 \partial #3}}
% \newcommand{\Di}[2]{\frac{\partial ^i #1}{\partial #2 ^i}}
% 
% 
% 
% %%%%%%%%% SHORT HAND %%%%%%%%%%
% \newcommand{\website}{\url{https://neurodata.io/}}
% \newcommand{\jhu}{Johns Hopkins University}
% \newcommand{\jvemail}{\href{mailto:jovo@jhu.edu}{jovo@jhu.edu}}
% \newcommand{\jv}{Joshua T.~Vogelstein}
% 
% \newcommand{\Vr}{V_{reset}}
% \newcommand{\Vl}{V_{leat}}
% \newcommand{\eqdef}{\overset{\triangle}{=}}
% \newcommand{\grad}{\nabla}
% \newcommand{\Hess}{\nabla\nabla}
% \newcommand{\defn}{\overset{\triangle}{=}}
% 
% \newcommand{\rto}{\leftarrow}
% \newcommand{\iid}{\overset{iid}{\sim}}
% \newcommand{\knn}{$k$NN}
% 
% \newcommand{\elegans}{\emph{C. elegans} }
% 
% \newcommand{\Lik}{\mathcal{L}}
% \newcommand{\Cae}{[\widehat{\text{Ca}}^{2+}]}
% \newcommand{\Cav}{\ve{C}}%[\ve{\text{Ca}}^{2+}]}
% \newcommand{\sml}{\sqrt{\ma{\lambda}}}
% \newcommand{\ml}{\ma{\lambda}}
% \newcommand{\nw}{\widehat{n}}
% \newcommand{\nv}{\vec{n}}
% \newcommand{\Ae}{\widehat{A}}
% \newcommand{\te}{\widehat{\tau}}
% \newcommand{\maxn}{\max_{\ve{n}: n_t \geq 0}}
% % \newcommand{\V}{\text{Var}}
% 
% \newcommand{\PmcP}{P \in \mc{P}}
% \newcommand{\mP}{\mathbb{P}}
% 
% % \newcommand{\dvs}{\dot{\bs}_t}
% % \newcommand{\dvw}{\dot{\bw}_t}
% % \newcommand{\dvx}{\dot{\bx}_t}
% % \newcommand{\dvy}{\dot{\by}_t}
% 
% \newcommand{\ft}{f_{\ve{\thet}}}
% \newcommand{\gt}{g_{\ve{\thet}}}
% \newcommand{\hht}{h_{\thetn}}
% 
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Ind}{\mathbb{I}}
% 
\newcommand{\wconv}{\overset{i.p.}{\rightarrow}}
\newcommand{\sconv}{\overset{i.p.}{\rightarrow}}
\newcommand{\conv}{\rightarrow}
\newcommand{\pconv}{\overset{p}{\conv}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\hatmcE}{\widehat{\mcE}}
\newcommand{\hatp}{\widehat{p}}
\newcommand{\hatP}{\widehat{P}}
\newcommand{\hatQ}{\widehat{Q}}
\newcommand{\hatL}{\widehat{L}}
\newcommand{\mhP}{\widehat{\PP}}
\newcommand{\tildeA}{\widetilde{A}}
\newcommand{\defeq}{\overset{\triangle}{=}}
% 
% 
% \DeclareMathOperator{\Pmat}{\mathbf{P}}
% \DeclareMathOperator{\veta}{\mathbf{\mb{v}}}
% \DeclareMathOperator*{\minimize}{\mathrm{minimize}}
% \DeclareMathOperator*{\maximize}{\mathrm{maximize}}
% % \DeclareMathOperator*{\mb{v}mod}{\mathbf{\mb{v}}}
% 
% 
% %%%%%%% LATIN LETTERS
% 
% 
% \newcommand{\bA}{\mb{A}}
% \newcommand{\bB}{\mb{B}}
% \newcommand{\bD}{\mb{D}}
% \newcommand{\bE}{\mb{E}}
% \newcommand{\bI}{\mb{I}}
% \newcommand{\bP}{\mb{P}}
% \newcommand{\bS}{\mb{S}}
% \newcommand{\bU}{\mb{U}}
% \newcommand{\bV}{\mb{V}}
% \newcommand{\bW}{\mb{W}}
% \newcommand{\bX}{\mb{X}}
% \newcommand{\bY}{\mb{Y}}
% \newcommand{\bZ}{\mb{Z}}
% 
% \newcommand{\ba}{\mb{a}}
% \renewcommand{\ba}{\mb{b}}
% \newcommand{\bd}{\mb{d}}
% \newcommand{\be}{\mb{e}}
% \newcommand{\bp}{\mb{p}}
% \newcommand{\bs}{\mb{s}}
% \newcommand{\bu}{\mb{u}}
% \newcommand{\bv}{\mb{v}}
% \newcommand{\bw}{\mb{w}}
% \newcommand{\bx}{\mb{x}}
% \newcommand{\by}{\mb{y}}
% \newcommand{\bz}{\mb{z}}
% 
% 
% \newcommand{\Aa}{\mathbb{A}}
% \newcommand{\BB}{\mathbb{B}}
% \newcommand{\CC}{\mathbb{C}}
% \newcommand{\DD}{\mathbb{D}}
% \newcommand{\EE}{\mathbb{E}}           % expected value
% \newcommand{\FF}{\mathbb{F}}
% \newcommand{\GG}{c}
% \newcommand{\HH}{\mathbb{H}}
% \newcommand{\II}{\mathbb{I}}           % indicator function
% \newcommand{\LL}{\mathbb{L}}
% \newcommand{\MM}{\mathbb{M}}
% \newcommand{\NN}{\mathbb{N}}
% \newcommand{\PP}{\mathbb{P}}
% \newcommand{\QQ}{\mathbb{Q}}
% \newcommand{\RR}{\mathbb{R}}
% \newcommand{\SSS}{\mathbb{S}}
% \newcommand{\VV}{\mathbb{V}}
% \newcommand{\WW}{\mathbb{W}}
% \newcommand{\XX}{\mathbb{X}}
% \newcommand{\YY}{\mathbb{Y}}
% \newcommand{\ZZ}{\mathbb{Z}}
% 
% 
% 
% 
% \newcommand{\Qs}{Q}
% \newcommand{\mcS}{\mc{S}}
% \newcommand{\mcU}{\mc{U}}
% 
% \newcommand{\mbd}{\ensuremath{\mb{d}}}
% \newcommand{\mbD}{\ensuremath{\mb{D}}}
% \newcommand{\mbx}{\ensuremath{X}}
% \newcommand{\mbX}{\ensuremath{\mb{X}}}
% \newcommand{\mby}{\ensuremath{Y}}
% \newcommand{\mbY}{\ensuremath{\mb{Y}}}
% 
% \newcommand{\mtbd}{\mtb{d}}
\newcommand{\mtbD}{\mtb{S}}
% \newcommand{\mtbx}{\mtb{x}}
% \newcommand{\mtbX}{\mtb{X}}
% \newcommand{\mtby}{\mtb{y}}
% \newcommand{\mtbY}{\mtb{Y}}
% 
% 
% 
% \DeclareMathOperator{\Ri}{\mathbf{\R}^{-1}}
% \DeclareMathOperator{\A}{A}
% \DeclareMathOperator{\W}{\mathbf{W}}
% \DeclareMathOperator{\V}{\mathbf{V}}
% %\DeclareMathOperator{\U}{\mathbf{U}}
% %\DeclareMathOperator{\C}{\mathbf{C}}
% \DeclareMathOperator{\uvec}{\mathbf{u}}
% \DeclareMathOperator{\D}{\mathbf{D}}
% \DeclareMathOperator{\Q}{\mathbf{Q}}
% \DeclareMathOperator{\R}{R} %\mathbf{P}}
% \DeclareMathOperator{\Y}{\mathbf{Y}}
% %\DeclareMathOperator{\BB}{\mathbf{B}}
% \DeclareMathOperator{\Hmat}{\mathbf{H}}
% \DeclareMathOperator{\Gmat}{\mathbf{G}}
% \DeclareMathOperator{\X}{\mathbf{X}}
% \DeclareMathOperator{\Cmat}{C} %\mathbf{L}}\providecommand{\ms}[1]{\mathsf{#1}}
% 
% \DeclareMathOperator*{\Ymod}{\mathbf{\Y}}
% \DeclareMathOperator*{\Bmod}{\mathbf{B}}
% \DeclareMathOperator*{\Hmod}{\mathbf{H}}
% \DeclareMathOperator*{\Lmod}{\mathbf{L}}
% \DeclareMathOperator*{\Xmod}{\mathbf{\X}}
% 
% 
% %%% THETA %%%%
% 
% \newcommand{\bth}{\ve{\theta}}
% \newcommand{\hth}{\mh{\theta}}
% \newcommand{\htth}{\mh{\theta}}
% \newcommand{\bhth}{\mh{\ve{\theta}}}
% \newcommand{\thetn}{\ve{\theta}}
% \newcommand{\thet}{\thetn}
% \newcommand{\theth}{\widehat{\ve{\theta}}}
% \newcommand{\theto}{\ve{\theta}'}
% \newcommand{\wht}{\widehat{\thet}}
% \newcommand{\wtt}{\widetilde{\thet}}
% \newcommand{\vth}{\ve{\thet}}
% \newcommand{\vTh}{\ve{\Theta}}
% \newcommand{\hvth}{\widehat{\ve{\thet}}}
% \newcommand{\bTh}{\ve{\Theta}}
% \newcommand{\hbth}{\widehat{\thet}}
% \newcommand{\tbth}{\tilde{\bth}}
% 
% 
% 
% % \newcommand{\p}{P_{\bth}}
% \newcommand{\pold}{P_{\bth'}}
% \newcommand{\pk}{P_{\widehat{\ve{\theta}}^{(k)}}}
% \newcommand{\pT}{P_{\thetn_{Tr}}} %\thetn_T
% \newcommand{\pO}{P_{\thetn_o}} %\thetn_o
% % \newcommand{\Q}{Q(\thetn,\theto)}
% % \newcommand{\m}{m^{\ast}}
% % \newcommand{\q}{q(\ve{H}_t)}
% \newcommand{\Ca}{[\text{Ca}^{2+}]}
% 
% 
% %%%%%% GREEK LETTERS
% 
\newcommand{\del}{\delta}
% \newcommand{\sig}{\sigma}
% \newcommand{\lam}{\lambda}
% \newcommand{\gam}{\gamma}
\newcommand{\eps}{\varepsilon}
% 
% \newcommand{\Del}{\Delta}
% \newcommand{\Sig}{\Sigma}
% \newcommand{\Lam}{\Lambda}
% %\newcommand{\Gam}{\Gamma}
% 
% \newcommand{\bSig}{\ve{\Sigma}}
% \newcommand{\bOm}{\ve{\Omega}}
% \newcommand{\bLam}{\ve{\Lambda}}
% \newcommand{\bPhi}{\ve{\Phi}}
% \newcommand{\bPsi}{\ve{\Psi}}
% 
% \newcommand{\bmu}{\ve{\mu}}
% \newcommand{\bal}{\ve{\alpha}}
% \newcommand{\bpi}{\ve{\pi}}
% \newcommand{\bkap}{\ve{\kappa}}
% \newcommand{\bdel}{\ve{\delta}}
% \newcommand{\bphi}{\ve{\phi}}
% \newcommand{\bpsi}{\ve{\psi}}
% 
% 
% 
% \DeclareMathOperator{\Delti}{\mathbf{\Delta}^{-1}}
% \DeclareMathOperator{\Delt}{Q} %\mathbf{\Delta}}
% \DeclareMathOperator{\Gam}{\mathbf{\Gamma}}
% \DeclareMathOperator{\Gami}{\mathbf{\Gamma}^{-1}}
% \DeclareMathOperator{\Sigb}{\mathbf{\Sigma}}
% 
% 
% \newtheorem{Def}{Definition}
% \newcommand\floor[1]{\lfloor#1\rfloor}

==> notes.tex <==
% jovo
- send to langford and naftali and shai shalev-shwartz

=========================
1. change mathcal{S}^n
2. clarify empty set use case for meta, zero shot learning
3. \mc{D}^n = {{s1,\cdot, s_n}:s_i \in \mc{S}} 
4. explicitly mention the necessity of decision problem

==> text/4_theoretical_results.tex <==
\section{Theoretical Results}

% In this section we establish a few simple theoretical results regarding the quantities we established earlier.
% % 
% Although it may seem obvious, one intuitively expects that from just out-of-task data, we should be unable to learn arbitrarily well. In the next result, we formally prove this intuition.

In this section we establish the relationship between our newly introduced generalized notions of learnability: weak, strong and non-uniform learnability, and consistency. 


\begin{proposition}[Strong implies weak]
    For an arbitrary task $t$, if we have strongly OOD learned at in-distribution sample size $n$, then we have weakly OOD learned at in-distribution sample size $n$.
\end{proposition}
\begin{proof}
    The proof follows very quickly from definitions. To have strongly OOD learned means that we can get arbitrarily close to optimal performance with arbitrarily high probability. To weakly OOD learn is to perform better than base performance $R_{XY}(\hat{h}_n)$ with arbitrarily high probability. Performing arbitrary well certainly implies performing better than base performance. Thus strong OOD learning implies weak.
\end{proof}
\begin{proposition}[Strong implies non-uniform]
    For an arbitrary task $t$, if we have strongly OOD learned at sample size $n$, then we non-uniformly OOD learned at sample size $n$.
\end{proposition}
\begin{proof}
    The proof also follows quickly from definitions. To have strongly OOD learned means that we can get arbitrarily close to optimal performance with arbitrarily high probability for all the distributions in the task model given a certain number of data points. To non-uniformly OOD learn means that we can get arbitrarily close to optimal performance with arbitrarily high probability for all the distributions in the task model given a certain number of data points that depends on the distribution. It is clear then that strong implies non-uniform since the number of data points required for the performance bound in strong OOD learning implies that this number of data points gives us the desired performance bound for all the distributions. This implies non-uniform OOD learning.
\end{proof}


Note that in the following results, meta-learning refers to scenarios in which we have in-distribution sample size $0$, i.e., zero data sampled from the evaluation distribution of a given task.


\begin{theorem}[Weak OOD ``Meta'' Learner Theorem] \label{thm:weak_metalearner_thm}
There exists tasks $t$ such that with zero data sampled from the evaluation distribution of that task, $f$ can weakly OOD learn, but $f$  does not strongly OOD learn. 
\end{theorem}

\begin{proof}
Consider the following scenario: The query space  is the unit interval, $\mc{X} = [0, 1]$. Each point $x \in \mc{X}$, is assigned a binary label (the action space $\mc{Y}$ is  $\{0, 1\}$). In other words, this is a simple realizable 0-1 classification task with zero Bayes error, $R^*=0$ (that is, there exists classifiers with no errors). Let the risk be the expected loss, where the loss is 0-1 loss. Let the hypothesis space be all functions $\mc{H} = \{h | h: [0, 1] \to \{0, 1\}\}$, and the learners be any learner.
    % 
    Consider distributions of the form
    \begin{align*}
        P(Y = y | X = x) & = \mathbb{I}(x \leq z)\mathbb{I}(y = 0) + \mathbb{I}(x > z)\mathbb{I}(y = 1),
    \end{align*}
    where $\mathbb{I}(a)$ is the indicator function that condition $a$ is true, $z \in [0, 1]$ and $X \sim U([0, 1])$.  Assume that the statistical model $\mc{P}_{X, Y}$ is the set of distributions where $z \in [0.7, 1]$.
    We will use $P_{z_0}$ to mean a distribution in $\mc{P}_{X, Y}$ with $z = z_0$. Assume we observe $n=0$ samples from the true but unknown $P_z \in \mc{P}_{X,Y}$.
    % 
    % Note that in this setting, $R^* = 0$.
    % 
    Further assume  that the data  pairs drawn according to $P_{\D}$ with the same form as distributions in $\mc{P}_{X, Y}$ but with $z = 0.6$. That is, $P_{0.6} \not\in \mc{P}_{X, Y}$, and thus we are in an OOD learning setting.
    % The error then is the expected risk in our case.
    
    This problem is weakly OOD learnable. For example, the learner that takes the biggest $x_0$ with label $0$ in the data and outputs hypotheses that labels any $x > x_0$ as $1$ and $0$ otherwise will perform better than chance with any desired probability $1 - \delta$ given enough data for any $P_{X, Y} \in \mc{P}_{X, Y}$.
    % 
    This setting is not strongly OOD learnable however. Assume for the sake of contradiction that we have some strong learner $f$ for this setting. Consider $P_{0.7} \in \mc{P}_{X, Y}$. If we let $\delta = \epsilon = 0.01$, then because $f$ is a strong OOD learner, there exists some $M$ such that with probability $1 - \delta = 0.99$, the learner outputs hypotheses whose risk only differs from the optimal risk by $\epsilon = 0.01$ whenever $m \geq M$.
    % 
    The risk here is calculated as
    \begin{align*}
        R_{P_{0.7}}(\hat{h}_{0, m}) = \int_{0}^{1}\mbb{I}(\hat{h}_{0, m}(x) \neq h^*_{0.7}(x))dx,
    \end{align*}
    where $h_{0.7}^*$, which outputs $0$ if $x \leq 0.7$, and $1$ otherwise, is the optimal hypothesis. $R_{P_{0.7}}(h_{0.7}^*) = 0$ in this scenario. Thus, by our assumption, $R_{P_{0.7}}(\hat{h}_{0, m}) < 0.01$ with probability greater than $0.99$. This implies that $f$ outputs hypotheses which differ from $h_{0.7}^*$ on at most $1\%$ of $[0, 1]$. 
    
    Now, take $P_{0.9} \in \mc{P}_{X,Y}$ as the task (in-) distribution and let $h^*_{0.9}$ be the optimal hypothesis for this distribution. Since the out-of-distribution data does not change, $f$ will output the same hypotheses as above for $m \geq M$. These hypotheses will differ from $h_{0.9}^*$ by more than $1 \%$ at least $99 \%$ of the time no matter how much out-of-task data we get (because they differ by at most $1 \%$ from $h_{0.7}^*$). In other words, at least $99 \%$ of the time, $R_{P_{0.9}}(\hat{h}_{0, m}) \geq \epsilon = 0.01$ no matter how high we make $m$.
    % 
    This contradicts $f$ being a strong OOD learner for the given setting, and so it is not strongly OOD learnable. That is, the setting is weakly OOD learnable but not strongly OOD learnable, which is the desired result.
\end{proof}

An immediate implication of the above theorem is that   the class of weakly OOD learning problems is larger than the class of strongly OOD learning problems. 

\begin{proposition}[Weak learning does not imply non-uniform learning]
    There are tasks $t$ for which weak OOD learning does not imply non-uniform OOD learning.
\end{proposition}
\begin{proof}
    The proof used for Theorem \ref{thm:weak_metalearner_thm} with small adjustments implies this result.
\end{proof}



% TODO non-uniform implies strong




==> text/5_supertasks.tex <==
% \section{Supertask Examples}
% \label{sec:supertask_examples}
\section{Learning Efficiency}
\label{sec:efficiency}

% The above definition of learnability is binary, that is, it enables one to ascertain \textit{whether} $f$ has learned, but not \textit{how much} $f$ has learned.  One could  directly leverage OOD learnability to obtain a learning amount (for example, for a fixed $\delta$ and $n$, what is $\eps$). 

With the definition of a generalized learning task in hand, a next natural question is whether a given learner $f$ has learned.  
Here, we build what we believe to be the simplest (and weakest) notion of learnability, which we term \textit{learning efficiency}, which we previously introduced in~\citet{pl}.  
Learning efficiency builds on the notion of relative efficiency from statistical estimation~\citep{bickel-doksum}.  In statistics, the relative efficiency of two different consistent estimators $f$ and $f'$ is the ratio of their variances (which is equal to the ratio of their generalization errors under certain assumptions). 
In contrast, learning efficiency evaluates the error of one particular learner $f$ as trained on two different datasets, $\D$ and $\D'$. 
% before and after acquiring data $\D_n$.  


\begin{definition}[Learning Efficiency]
     The learning efficiency $(\LE)$ for task $t$ with learner $f$ is a function
    % \begin{align*}
        $\LE^t_f: \mc{S}^* \times \mc{S}^* \to \mathbb{R}$
        % .
    % \end{align*}
        % Specifically, learning efficiency for task $t$ 
        is defined by
    \begin{align*}
        \LE^t_f(\D, \D') 
        = \frac{\mc{E}^t_f(\D)}{\mc{E}^t_f(\D')}, 
    \end{align*}
    where each expectation in the error is taken with respect to the corresponding data set distribution, i.e. the numerator expectation is taken with respect to the distribution governing $\D$, and the denominator expectation is taken with respect to the distribution governing $\D'$.
\end{definition}


We say that $f$ has learned more about task $t$ leveraging data $\D'$ as compared to $\D$ whenever 
$\LE^t_f(\D, \D' ) >1$, 
% $\LE^t_f(\emptyset, \mb{B}) >1$, 
or equivalently, whenever $\log \LE^t_f(\D, \D' ) >0$.
% , which we refer to as positive transfer (from data set $D^B$ for task $t$ by learner $f$). 
In this manuscript, we are typically interested in cases where $\D$ is a strict subset of $\D'$. In such scenarios, positive (log) learning efficiency indicates that the learner was able to successfully transfer information (that is, learn) from the elements of $\D'$ not in $\D$, $\D' \backslash \D$, to improve performance on task $t$.  
This definition of learning immediately implies a definition of \textit{forgetting}: 
$f$ has forgotten about task $t$ leveraging data $\D'$ as compared to $\D$ whenever
$\log \LE^t_f(\D, \D \cup \D') <0$. While interference and forgetting are often discussed  in  articles about both natural and artificial intelligence~\citep{McCloskey1989-nl,kirkpatrick2017overcoming}, we have never seen a formal definition of forgetting in the literature. 


Learning efficiency is therefore a function of $\D$ and $\D'$ for any given samples sizes, $n$ and $m$, respectively  (it may be the case that $n=0$ and/or $m=0$). Given the two distributions describing $\D$ and $\D'$, one could plot a two-dimensional surface of learning efficiency as a function of $n$ and $m$. This would completely characterize the learning efficiency for the given task.
An increase in learning efficiency corresponds to an increase in the degree $f$ learns from $\D'$ as compared to $\D$ for task $t$. \todo{Does $S$ and $S'$ belong to different task distributions? Or is it a more general definition? Data Models paper by Alexander Madry also discusses something similar. I think it would be good to discuss some limitations of LE in this draft? e.g. It can compare the effect of only two datasets at a given time.}

Implicit in this definition is that the $f$ in the numerator and the $f$ in the denominator are operating on the same hyperparameter, $\lambda$. In some cases, the hyperparameter $\lambda$ could be a function of the sample size, for example, if sample size is small, $\lambda$ penalizes more.  In that case, we would write $\lambda_n$ as the penalty for sample size $n$, and we would require that the sequence $\mb{\lambda} = \lambda_1, \lambda_2, \ldots$ would be the same sequence  in the numerator and denominator.
% 
Evaluating this ratio therefore requires training and evaluating the exact same $f$ \textit{twice}: once with $\D$, and once with  $\D'$.
% 
If this ratio is bigger than $1$ (or, equivalently, its log is positive), then we say that $f$ \textit{learned} from $\D'$---over and above that which $f$ learned via simply $\D$---with respect to task $t$.  
Learning efficiency thus allows us to measure the extent to which  $f$ leverages the data $\D'$ to improve performance on task $t$. 
% 

We note that these definitions of learning and forgetting are ``global'', in the sense that, in expectation, the risk of the hypothesis after learning  improved over the risk prior to the additional data.  In other words, these definitions perform an average over the entire space, rather than being restricted to any one part of the space. Note that because this is an average, one can also locally learn even if one does not globally learn. Imagine for example, that the induced hypothesis improved its risk in some subspace of the query space $\mc{X}' \subsetneq \mc{X}$, but got worse (aka, forgot) in another subspace $\mc{X}'' \subsetneq \mc{X}$, where $\mc{X}' \cap \mc{X}'' = \emptyset$. In such a scenario, depending on $P_{X,Y}$, it could be that expected risk (i.e. the risk averaged over the entire space) got worse, in which case, overall learning efficiency would be log negative.  So, in this scenario, $f$ locally learned and globally forgot. 


As noted above, in learning efficiency, there is no minimum sample size. Rather, one can compute learning efficiency for any $n,m \geq 0$. 
Thus, zero-shot and few-shot learning are perfectly fine notions of learning that can be theoretically and empirically investigated via studying learning efficiency.
This is in stark contrast to in-distribution definitions of learning, all of which require a sufficiently large sample size  to ascertain whether $f$ has learned.  


\section{Formalizing distinct learning paradigms}
\label{sec:hier}

In this section we apply our notion of learning efficiency to characterize whether, and the extent to which, a learner has learned in various different learning scenarios.  We made a number of choices based on the literature to formalize these learning scenarios, some of which are not universally agreed upon.  That said, the names of the different learning scenarios are only important for clarity of communication; our main intent with this section is to illustrate the flexibility of our proposed formalism.
% % \paragraph{Task Awareness} \label{sec:task_aware_decisions}

We reiterate again from earlier: we are typically interested in cases where the in-distribution data set, $\D$, is a strict subset of the out-of-distribution data set, $\D'$. In such scenarios, positive (log) learning efficiency indicates that the learner was able to successfully transfer information (that is, learn) from the elements of $\D'$ not in $\D$, $\D' \backslash \D$, to improve performance on task $t$. As this section proceeds forward, note the common thread of the learning efficiency taking the form $\LE(\D, \D')$, where $\D \subset \D'$.

 


\subsection{In-distribution learning}

In-distribution learning is the simplest learning scenario. It includes as special cases hypothesis testing, point estimation, unsupervised learning, supervised learning, federated learning, online learning, forecasting, games, and reinforcement learning.  
% Recall that $\D_0$ is the ``data set'' prior to observing $\D_n$, which may include inductive biases, priors, previously learned models, etc.


Let $h_0$ be the hypothesis output by the learner prior to seeing $\D_n$. In the \textit{tabula rasa} learning mentality (that is, where learning happens upon a blank slate~\citep{Pinker2003-sh}), $h_0$ would be the hypothesis prior to seeing \textit{any} data.  However, more generally, it is simply the hypothesis prior to seeing a new data set, $\D_n$.  We define $\D_0$ to be the `data set' prior to seeing $\D_n$, which might be the empty data set, and we let $f(\D_0)=h_0$ denote the `base hypothesis'.  
$\D_0$ can be quite general; specifically, $\D_0$ \todo{$h_0$? $S_0$ is more like a notion of dataset, I suppose?} could be a hypothesis learned from a previous data set, or a prior obtained from another data set, etc. (recall that our definition of the data sample space $\cS^*$ above was  unrestricted). 
% 
$h_0$ is therefore a function of the inductive bias of the learner $f$, as well as its hyper-parameters, and `initial conditions' (such as the randomization of the weights prior to training a deep network), as well as anything else learned from $\D_0$.  Note that $h_0$ may, in general, also be a random variable, though we ignore that source of variability here. $h_0$ could also be the na\"{i}ve chance hypothesis, which assumes a non-informative prior on the action space.
From a Bayesian perspective, $\hat{h}_0$ corresponds to our prior knowledge for how to respond to a given query, and $\hat{h}_n$ corresponds to our posterior updated knowledge, based on data set $\D_n$. 



\begin{application}[Learning Efficiency for In-Distribution Learning]\label{def:le}
    The \textbf{learning efficiency} of an in-distribution  learner $ f $ for task $t$ given data sets $\D_n$ is the learning efficiency for task $t$ with a $\D = \D_0$ and $\D' = \D_n$,
    \begin{align*}
        \LE_f^t(\D_0, \D_n) & = \frac{\mc{E}_f^t(\D_0)}{\mc{E}_f^t(\D_n)} \enspace.
    \end{align*}
    We say that $f$ learns in this task with $n$ samples if $\log \LE_f^t > 0$.
\end{application}

This definition has conditioned on a particular sample size, $n$.  One could generalize this definition to be a function of $n$, and define the learning efficiency curve for a given learner $f$ on this task.  


\subsection{Transfer Learning}
\label{sec:formal_transfer}
Transfer learning is arguably the simplest OOD learning scenario with one underlying task $t$ along with an explicit set of $J$ data sets $\{\D^1, \dots, \D^J\}$~\citep{Pratt1993-yn, Pan2010-bv}.  
% 
$\D^1$ here is data associated with task $t$, often called the \textit{target data} (though we call it the `in-distribution' data throughout for clarity); 
that is, it is assumed to be drawn according to the evaluation distribution for task $t$. 
Without loss of generality, we assume that $\D^1$ includes the base data set, $\D_0$, that is, $\D_0 \subset \D^1$ 
(thus, $|\D^1| \geq 1$, because it always includes $\D_0$ at least).
 The other data sets, $\D^2, \dots, \D^J$---sometimes called side information~\citep{Shannon1958-no}, or `source data'---are available to assist in learning and producing a better hypothesis (we refer to these data as the `out-of-distribution data' for clarity). 
%  Note that we may have $\abs{\D^1} = 1$ (because at minimum $\D_1$ includes $\D_0$).
% or for any $m = 1, 2, \dots, M$. 
% TODO@ali what is the point of letting the other data sets be empty? @jovo from ali: I was thinking about it as transfer learning is a pure generalization of regular learning. I agree you're not really transferring anything if the out-of-task data sets are empty though.
Let $\D_n = \bigcup_{j = 0}^{J}\D^j$ be the amalgamated data set. %, which includes $\D_0$, the potentially empty base data set.
% 
While the problem associated with this task is  to produce a hypothesis that minimizes the  risk for task $t$; the fundamental question in transfer learning is whether a learner has successfully leveraged the out-of-distribution (or source) data to improve performance. That is, has the {\it generalization error  decreased} by virtue of leveraging $\D^2, \dots, \D^J$, relative to only using $\D^1$?

To answer such a question, we consider the performance $\mc{E}_f^t(\D^{1})$ of the hypothesis learned by $f$ using only task $t$ data, as compared to  the hypothesis learned by  $f$ using all the data $\mc{E}_f^t(\D_n)$. 
% We evaluate the {transfer efficiency} of a transfer learner as defined below.
\begin{application}[Learning Efficiency for Transfer Learning]\label{def:te_for_tl}
    The \textbf{transfer learning efficiency} of a transfer learner $ f $ for task $t$ given data sets $\D=\{\D^1, \dots, \D^J\}$ is the learning efficiency for task $t$ with a $\D = \D^1$ and $\D' = \D_n$,
    \begin{align*}
        \LE^t_f(\D^1, \D_n) & = \frac{\mc{E}^t_f(\D^1)}{\mc{E}^t_f(\D_n)} \enspace.
    \end{align*}
    We say that $f$ transfer learns in this supertask if $\log \LE^t_f > 0$.
\end{application}
The above definition is identical to the definition of learning efficiency, where  $\D=\D^1$ and $\D'=\D_n$. In other words, transfer learning is  a generalization of in-distribution learning (when $\D^1 = \D_0$). Stated differently,  in-distribution learning is a special case  of transfer learning, but in-distribution learning transfers from priors and inductive biases rather than out-of-distribution data. \todo{Just a suggestion: May be as an example, we can explain how pretraining-finetuning (the most popular TL method used in practice for deep nets) fits into this definition.}
  

While others often include a `source task' in defining transfer learning, in our definition, we only specify one task, that is, the `target task'. Source (out-of-distribution) data may have a source task associated with it, but from the perspective of optimizing learning efficiency for the target task, there is no need to  specify a source task with its associated risk, etc.  
% 
Note that we have conditioned on the sample size for all data sets. Doing so enables us to avoid making any assumptions about the total number of possible data sets, or the distribution over those data sets. One could define a notion of learning efficiency with respect to a distribution over data sets and sample sizes, and take additional expectations to obtain something like expected learning efficiency.  


\subsection{Multitask Learning}
\label{sec:formal_multi}
Multitask learning can be thought of as a generalization of transfer learning~\citep{Bengio1992-pe, Caruana1997-mm}. Assume the existence of an \textbf{environment} of  tasks $\mc{T}$, with cardinality $|\mc{T}|$, along with $J$ data sets $\mc{J}=\{\D^1, \dots, \D^J\}$.
% 
We  let $\D_n$ be all of the data (i.e. the amalgamated data set as defined above, including the base data). 
For simplicity of presentation, and without loss of generality, we assume that all of the tasks share a common data space, query space, action space, etc.; that is, the tasks share a common setting. The tasks can differ on the data sets that come with them, their  distributions,  risks, and errors. 
% 
Let $\D^t$ be the data associated with task $t \in \mc{T}$ drawn according to the data distribution of task $t$. 
Note that it is possible that $J \geq |\mc{T}|$. Of course, the data set $\D_t$ associated with a given task $t$ may have no data, in which case we have no in-distribution data for that task. 
Any data set $\D^t$ with $t > |\mc{T}|$ is not associated with any specific task.
It could be the case that a given data set is associated with multiple tasks; in that case, we simply `copy' the data set as many times as necessary to ensure there that each task has one data set associated with it. 
Just like in transfer learning, we want to measure whether performance improves on each task by virtue of seeing out-of-distribution data. 
% In a slight abuse of notation, 
Let $\mc{E}_f^t(\D^t)$ denote the generalization error of the hypothesis learned by $f$ on task $t$ using only the data associated with that task, $\D^t$.  
For notational simplicity, we assume each of $\D^t$ includes the base data $\D_0$, that is, $\D_0 \subset \D^t$.  
And let $\mc{E}_f^t(\D_n)$ denote the generalization error of the hypothesis learned by $f$ on task $t$ using all available data,  $\D_n$. Now, we can define multitask learning efficiency.

% The performance of the learner on task $t$ consuming only task $t$ data is $\mc{E}_f^t(\D^t)$, while the performance of the  learner on task $t$ using all available data is $\mc{E}_f^t(\D)$. The superscript $k$ indicates that we use the risk from task $t$ in evaluating the generalization error, $\mc{E}_f^t(\cdot)$. Hence we can index learning efficiency in this context by $k$.
% 
\begin{application}[Learning Efficiency for Multitask Learning]
The \textbf{multitask learning efficiency} of $ f $ for tasks $\mc{T}$ given data sets $\mc{J}$ is the set of learning efficiencies with the task $t$ risks, with $\D = \D^t$, and $\D' = \D_n$,
 \begin{equation*}
    \LE_f^t(\D^t, \D_n) = \frac{\mc{E}_f^t(\D^t)}{\mc{E}_f^t(\D_n)}, \qquad t \in \mc{T}.
    \label{eqn:te_t}
\end{equation*}
    In other words, in multitask learning, we have a set of $|\mc{T}|$ learning efficiencies, one for each of the tasks. 
\end{application}

Note that this is another instance of learning efficiency, with $\D$ and $\D'$ denoting different data sets. 
The multitask setting naturally leads to questions about performance \textit{across} tasks. To quantify learning across tasks we introduce a non-negative weight per task, $\mb{w}=(w_1, w_2, \ldots)$, where $\sum_{t \in \mc{T}} w_t = 1$.  
% Did we multitask learn on average? Did we multitask learn for each task? These questions lead us to  the following definition.

\begin{application}[Multitask Learning]
    Learner $ f $ $\mb{w}$-multitask learns if the log of the convex combination of learning efficiencies of each task is positive. That is, $f$ multitask learns if 
    \begin{align*}
        \log \sum_{t \in \mc{T}} w_t \cdot \LE_f^t(\D^t, \D_n) > 0 \enspace .
    \end{align*}
    %  where $\mb{w}=(w_1,\ldots, w_K)$ is a specified set of non-negative weights that sum to $1$.
\end{application}

The advantage of having a general set of weights is that it allows a varying measure depending on the situation. For example, we may have multiple tasks but only care about transfer to one task. In that case, all of the weight would be placed on the learning efficiency of that task, and we are back to the case of transfer learning with one task. The other tasks' data can then be  thought of as just more buckets of side information. This shows that multitask learning is a generalization of transfer learning. 
% 
Alternatively, if  we let $w_t = 1/|\mc{T}|$ for all $t \in \mc{T}$, then we have a version of multitask learning that could be considered \textit{weak multitask learning}.  
In this scenario, we say $f$ has multitask learned whenever the log of the \textit{average} learning efficiency is positive. 
A learner $f$ strong multitask learns in an environment $\mc{T}$ whenever it $\mb{w}$-multitask learns for any feasible vector of weights $\mb{w}$. An immediate implication of strong multitask learning is that $f$ positively transferred for \textit{all} tasks in the environment, that is, each task has benefited from the out-of-distribution data. 
% 
In general, for any set of weights $\mb{w}$, if a learner multitask learns, it has necessarily transfer learned for at least one of the $|\mc{T}|$ tasks.


\subsection{Meta-Learning}\label{sec:meta_learning}
% 
In practice, meta-learning is very related to multitask learning. Again, assume we have an environment $\mc{T}$, but unlike in typical multi-task learning scenarios the cardinality of the environment, $\abs{\mc{T}}$, could be infinite.
And further assume that we have already faced $K$ of the tasks, and label the set of already observed tasks $\mc{T}_K$.  
As before, we have $J$ data sets, $\{\mb{S}^1,\ldots, \mb{S}^J\}$, where $J \geq |\mc{T}_K|$.
Now, we face a  
task, $t$ which may or may not be an element of $\mc{T}_K$ and acquire a new data set, $\mb{S}^{J+1}$. 
% 
% and a sub-environment $\mc{T}_k$ such that $\mc{T}_k \subset \mc{T}_n$. Assume the same set up as multitask learning. Also assume, however, that we get access to data from that sub-environemnt. That is, with the set of data sets $\{\D^1, \dots, \D^m\}$, we only get access to $\D^1, \dots, \D^t$, and $\D^{n + 1}, \dots, \D^m$, where $k < n \leq m$.
% 
% We are now confronted with a task from $\mc{T}_m\setminus\mc{T}_k$. 
The question of meta learning is, did learning tasks $\mc{T}_K$ using data $\{\mb{S}^{j}\}_{j = 1}^{J}$ help us learn more efficiently for task $t$? Intuitively, we we want to measure if we learn task $t$ more efficiently with  $\mc{J} = \{\mb{S}^1,\mb{S}^2, \ldots, \mb{S}^{J+1}\}$, as compared to learning task $t$ with just $\mb{S}^{J+1}$. 
The new data may arrive with complete task information (i.e., the task aware learning setting), no task information (i.e., the task unaware or agnostic learning setting), or partial information (i.e., the task semi-aware learning setting). 
% 
% 
As in multitask learning, a weight is associated to each task $\mb{w} = \{w_1, w_2,   \dots\}$ over all $t  \in \mc{T}$. We further constrain the weights to form a discrete probability distribution, that is, $\sum_{i = 1}^{\infty}w_i = 1$, $w_i \geq 0$.



\begin{application}[Meta-Learning]
    Learner $ f $ $\mb{w}$-meta-learns in environment $\mc{T}$ using data set $\mc{J}$ if 
    \begin{align*}
    \log \sum_{t \in \mc{T}} w_t \cdot \LE_f^t(\D^t, \D_n) > 0.
\end{align*}
    % the convex combination of learning efficiencies of each subtask is greater than $ 1 $. That is,
    % \begin{align*}
    %     \sum_{k = 1}^{K} w_k \cdot \LE_f^t(\D^t, \D) > 1,  
    % \end{align*}
    %  where $\{w_k: j = 1, \dots, K\}$ is some set of non-negative weights whose sum is $1$.
\end{application}


The implication of the above definition is that if $f$ has $\mb{w}$-meta-learned, then, it will perform better on tasks in the environment than it would have if it had not observed the previous $K$ tasks and $J$ data sets. If $\mc{T} = \mc{T}_K$, then meta-learning is simply multitask learning, indicating that meta-learning is a generalization of multitask learning. The key difference between the two is in meta-learning there are unobserved tasks, whereas in multitask learning, the learner has \textit{a priori} access to all tasks. 
Weak meta-learning, like weak multitask learning, corresponds to the setting where the log of the \textit{average} learning efficiencies is positive.  Strong meta-learning, like strong multitask learning, corresponds to the setting where the log of each learning efficiency is positive, that is, $f$  positively transfers for each task in the environment. 
Note that sometimes meta-learning is defined in a similar fashion, except that $t \notin \mc{T}_K$, such that $f$ learns faster specifically on \textit{new} tasks.  

Our definition of meta-learning generalizes  Baxter's in a few ways~\citep{Baxter2000-wv}. First, Baxter did not allow for additional out-of-distribution data sets, rather, there was a one-to-one mapping between data sets and tasks. Second, Baxter was only interested in hypotheses that performed well for any distribution in the environment, akin to our strong meta-learning.  


\subsection{Continual Learning}\label{sec:continual}
Continual learning generalizes multi-task and meta-learning, and therefore, some variants of it are referred to as online meta-learning~\citep{Finn2019-yv}. 
There are two key points of departure.  First, in meta-learning, we did not assume a distribution over tasks, rather, just a weight assigned to how much one cares about a task. In continual learning, tasks are governed by a (potentially non-stationary and even adversarial) stochastic process, akin to  the  random processes governing the data in online learning (see \citet{Shalev-Shwartz2010} for more details).  Second, unlike meta-learning, but like streaming learning, continual learning necessarily includes  computational complexity constraints (which are often not explicitly enumerated)~\citep{pl}, as described below.

% 
Several works have explored this scenario as well as presented novel learners for it~\citep{Aljundi2019, Zeno2019, He2020, Lee2020}. Here we formalize the framework they explored using the above established conventions.
% 
In the most general version of continual learning, we have streaming data, queries, actions, error, and \textit{tasks}---in contrast to in-distribution online learning, where the task is fixed \textit{a priori}. We assume that each (data, queries, actions, error, and tasks) is governed by a stochastic process.
% 
While in online learning, sequential learning, and reinforcement learning, only the distribution of the data may change, in continual learning, other aspects of the task may also be dynamic.  
In other words, in other learning scenarios the setting is fixed; in contrast, in continual learning, the setting can dynamically (and even adversarially) change. 
Hence, anything about a task can change in any moment (although the learner might not be aware of everything that has changed). 
% 
A particularly interesting and special case of continual learning occurs when the data arrive in batches from the same task. 
% that arrive sequentially all come from the same task, 
% in which case we have the common online meta-learning and/or multitask learning problems.  % \comE{This is online MTL -- there are other forms of lifelong ML.}
% The above description of rounds implicitly depends on the existence of a task -valued stochastic process, to complement the data, query, action, and feedback processes. 

A second distinction between continual learning learning and some sequential learning scenarios is that continual learning necessarily includes computational complexity constraints~\citep{Van_Rooij2019-hu}.  If it did not, then the learner $f$ (or hypothesis $h$) could store all the data $\D_n$, and retrain everything from scratch.  Such a strategy would na\"ively require $\mc{O}(n)$ space and $\sum_{i=1}^n i = \mc{O}(n^2)$ time (assuming each data sample is the same size). 
Therefore, a \textit{bona fide} continual learner must, at a minimum, have a computational upper bound of  $o(n)$ space and/or $o(n^2)$ time, and should in practice be far more efficient. 

Intriguingly, many previously proposed purported continual learners do not satisfy the above mentioned computational complexity constraints. \citet{pl} quantifies the complexity of several state-of-the-art claimed continual learners, and shows that  Elastic Weight Consolidation~\citep{kirkpatrick2017overcoming} and Progressive Neural Networks~\citep{Rusu2016-zm} fail to satisfy the computational complexity constraints established above, rendering them not \textit{bona fide} continual learning algorithms (although some generalizations of them both do satisfy these criteria).  

As mentioned above, for the formalism described in \S \ref{sec:gen_learnability} to account for continual (and lifelong) learning, it must be generalized somewhat to replace the random variables with stochastic processes, incorporate a stochastic process on tasks, and generalize the class of learners to include updating hypotheses. 





\paragraph{Quantifying continual learning}
The first thing we have to do is make adjustments to the framework as necessary to account for the nature of continual learning. Mainly, the form of the error has to be adjusted. 
% 
% 
% 
In a continual learner, the learner lives in continuous time, and every once in a while, it receives data. Its data is updated, $\D_{n-1} \rightarrow \D_n$. The learner gets to interpret the data as previous query-action pairs, (potentially noisy) error, and/or side information, such as a particular setting or task label. After acquiring new data, the learner updates its hypothesis, and interprets the input as a query $f(\D_n, \mh{h}_{n-1}) \rightarrow (X_n, \mh{h}_{n})$.  This hypothesis then chooses  an appropriate action (including no action) based on that presumed query, $\mh{h}_n(X_n) = Y_n$. In the case when we have a loss, the error then looks like

\begin{equation}
\begin{split}
 \sum_{n=n'}^m w_n \int_{\mc{S}_n}  \int_{(\cX_n, \cY_n)} \ell_n(\hat{h}_n(X_n), Y_n) dP_{(X_n,Y_n,T_n) | \D_n } dP_{\D_n}
    \enspace , 
\end{split}
\end{equation}
\todo{Looks like this definition misses some clarity. For instance, what is $n', m,$ and $T_n$?}
\noindent
where the $n$ subscript indicates we are at time $n$. So $\ell_n$ is the loss at the $n$th data reception, $\D_n$ is the updated data, $\hat{h}_n$ is the new hypothesis at that time, $\cX_n$ is the query space at that time, and so on.
% 
Thus we measure the performance of our learner not only on the current task but on future tasks as well.

New quantities of interest arise as well due to the sequential nature of learning in this environment. For example, how much do past tasks help us in learning for the current task? How much do future tasks help us in learning for the past tasks? These questions lead us to define  evaluation criteria (informally introduced  in~\citet{pl}). First, given a task of interest $t$, we define $\D^{< t}$ to be the set of data points up to and including the last data point from task $t$. 
% Let $\D_n$ be all of the data. %We can now define the following.
% \comE{Need to distinguish vs meta-learning}
% 
% For the first posed, we introduce the following quantity,
\begin{application}[Learning Efficiency for Forward Transfer]
The \textbf{forward learning efficiency} of $ f $ for task $t$ given $ {n} $ samples is the learning efficiency with the task $t$ risk, $\D = \D^t$, and $\D' = \D^{< t}$,
\begin{align}
    \LE_f^t(\D^t, \D^{< t})
\end{align}
We say that $f$ forwards learns if the forward learning efficiency is greater than $1$, or equivalently, if $\log \LE_f^t > 0$. 
% $\LE_f^j$ indicates that we are using the task $t_j$ risk.
\end{application}

% As for the second posed question, we introduce the following quantity,


\begin{application}[Learning Efficiency for Backward Transfer] 
The \textbf{backward learning efficiency} of $ f $ for task $t $ given $ {n} $ samples is the learning efficiency with the task $t$ risk and $\D = \D^{< t}$ and $\D' = \D_n$,
\begin{align}
    \LE_f^t(\D^{< t}, \D_n)
\end{align}
We say that $f$ backward learns if the backward learning efficiency is greater than $1$, or equivalently, if $\log \LE_f^t >0$. 
% $\LE_f^j$ indicates that we are using the task $t_j$ risk. 
\end{application}

Note that this concept of backward transfer is closely related  to ``reverse transfer'' which was first introduced in~\citet{Ruvolo2013-hk}.
% 
Multiplying forward and backward transfer efficiency for a particular task recovers learning efficiency for that task: 
\begin{align*}
    \LE_f^t(\D^t, \D) & = \LE_f^t(\D^t, \D^{< t}) \times \LE_f^t(\D^{< t}, \D) \enspace .
\end{align*}

Putting all the above together, we can now define whether $f$ has continually learned. As before with meta-learning, we assume that the weights form a discrete probability distribution.

\begin{application}[Continual Learning]
    Learner $ f$ $\mb{w}$-continually learns tasks $t \in \mc{T}$ if the log of the convex combination of learning efficiencies  is greater than $0 $. That is, $f$ $\mb{w}$-continually learns if 
    \begin{align*}
        \log \sum_{t \in \mc{T}} w_t \cdot \LE_f^t(\D^t, \D) > 0 \enspace .   
    \end{align*}
    %  where $\{w_k\}_{k \in [K]}$ is a specified set of non-negative weights that sum to $1$.
\end{application}

Weak and strong continual learning are defined as in weak and strong multitask and meta-learning. If one sets the weights of all the unobserved tasks to zero, then continual learning above corresponds to continual \textit{multitask} learning.  On the other hand, allowing the weights of unobserved tasks to be positive, then the above corresponds to continual \textit{meta-}learning.  It may sometimes be desirable to assert that $f$ continually learns only if it achieves positive forward and backward $\mb{w}$-learning efficiency. 

\subsection{Lifelong Learning}\label{sec:lifelong}

While others have used the terms continual and lifelong learning interchangeably, here, we argue that there can be important meaningful differences between the two. 
Specifically, we advocate that lifelong learning is a generalization of continual learning that renders it closer to biological learning.  The key difference between lifelong learning and continual learning is that in lifelong learning, two things can change over the lifetime of the agent.  First, the weights on each task may vary over time.  In continual learning, the weights are typically specified \textit{a priori}, and are fixed over the duration of learning.  In contrast, in lifelong learning, the value of any individual task may change over time.  For example, frogs do not need to know how to swim as tadpoles after they metamorphose, so the weight on swimming as a tadpole goes down to zero at that point.  
Second, the computational constraints can change over the lifetime of the learner.  Specifically, learners essentially go through three life phases. First, while the learner is juvenile, it can increase its resources as more data and tasks are presented to it. In this phase, it builds representational capacities.  Second, while the learner is an adult, it has fixed resources, and therefore, must leverage and recombine existing resources to obtain new capabilities, but cannot grow new resources.  Third, while the learner is a geriatric, it has diminishing resources, and therefore, must re-prioritize its allocation of resources to ensure that it does not forget crucial skills (such as how to breath).  These resource constraints can be expressed in terms of the sets of hypotheses and learners under consideration at each time. 
To our knowledge, there are no existing algorithms that currently can satisfy these additional complications, despite the fact that all biological learning agents must address them. 
Let $w_{t,u}$ correspond to the weight on task $t$ at time $u$, so $\mb{w} = ( w_{t,u} )$, and let
$\LE_f^{t,u}$ denote the learning efficiency for task $t$  that may be changing with $u$. 
% 
% For the most part, the literature has not clearly differentiated between what we refer to as continual and lifelong learning here. 

\begin{application}[Lifelong Learning]
    Learner $ f $ $\mb{w}$-lifelong learns tasks $t \in \mc{T}$ if the log of the convex combination of learning efficiencies   is greater than $0$. That is, $f$ $\mb{w}$-lifelong learns if 
    \begin{align*}
        \log \sum_{u > 0} \sum_{t \in \mc{T}} w_{t,u} \cdot \LE_{f}^{t,u}(\D^t, \D) > 0 \enspace .   
    \end{align*}
    %  where $\{w_k\}_{k \in [K]}$ is a specified set of non-negative weights that sum to $1$.
\end{application}

